Quantifying the Knowledge in a DNN to Explain Knowledge Distillation for Classification

Compared to traditional learning from scratch, knowledge distillation sometimes makes the DNN achieve superior performance. This paper provides a new perspective to explain the success of knowledge distillation, i.e., quantifying knowledge points encoded in intermediate layers of a DNN for classification, based on the information theory. To this end, we consider the signal processing in a DNN as the layer-wise information discarding. A knowledge point is referred to as an input unit, whose information is much less discarded than other input units. Thus, we propose three hypotheses for knowledge distillation based on the quantification of knowledge points. 1. The DNN learning from knowledge distillation encodes more knowledge points than the DNN learning from scratch. 2. Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. In comparison, the DNN learning from scratch tends to encode various knowledge points sequentially. 3. The DNN learning from knowledge distillation is often optimized more stably than the DNN learning from scratch. In order to verify the above hypotheses, we design three types of metrics with annotations of foreground objects to analyze feature representations of the DNN, \textit{i.e.} the quantity and the quality of knowledge points, the learning speed of different knowledge points, and the stability of optimization directions. In experiments, we diagnosed various DNNs for different classification tasks, i.e., image classification, 3D point cloud classification, binary sentiment classification, and question answering, which verified above hypotheses.

==> distill latex/distill_check.tex <==



\section{abstract}
Compared to traditional learning from scratch, knowledge distillation sometimes makes the DNN achieve superior performance.
This paper provides a new perspective to explain the success of knowledge distillation, \textit{i.e.} quantifying knowledge points encoded in intermediate layers of a DNN for classification, based on the information theory.
To this end, we consider the signal processing in a DNN as the layer-wise information discarding.
A knowledge point is referred to as an input unit, whose information is much less discarded than other input units.
Thus, we propose three hypotheses for knowledge distillation based on the quantification of knowledge points.
\textbf{1.} The DNN learning from knowledge distillation encodes more knowledge points than the DNN learning from scratch. 
\textbf{2.} Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. In comparison, the DNN learning from scratch tends to encode various knowledge points sequentially.
\textbf{3.} The DNN learning from knowledge distillation is often optimized more stably than the DNN learning from scratch.
In order to verify the above hypotheses, we design three types of metrics with annotations of foreground objects to analyze feature representations of the DNN, \textit{i.e.} the quantity and the quality of knowledge points, the learning speed of different knowledge points, and the stability of optimization directions. 
In experiments, we diagnosed various DNNs for different classification tasks, \textit{i.e.} image classification, 3D point cloud classification, binary sentiment classification, and question answering, which verified above hypotheses.





\section{Introduction}
Knowledge distillation has achieved great success in various applications.
Knowledge distillation is referred to as the process of transferring the knowledge from one or more well-trained deep neural networks (DNNs), namely the teacher networks,
to a compact-yet-efficient DNN, namely the student network.
However, there have been very few studies to explain how and why knowledge distillation outperforms traditional learning from scratch.

Hinton owed the superior performance of knowledge distillation to the use of ``soft targets''.
Furlanello conjectured the effect of knowledge distillation on re-weighting training examples.
Lopez-Paz interpreted knowledge distillation as a form of learning with privileged information. 
Besides, from the perspective of network training, knowledge distillation was regarded as a label smoothing regularization method, and could enable faster convergence. 
These explanations for knowledge distillation were mainly based on qualitative statements or focused on the optimization and regularization effects.

Beyond the above perspectives for explanations, this paper provides a new perspective to analyze the success of knowledge distillation, \textit{i.e.} quantifying knowledge points encoded in the intermediate layer of a DNN. 
In other words, the quantity of knowledge points and the quality of knowledge points enable us to explain the representation power of the DNN, which is trained for classification.
For a better understanding, let us take the image classification as an example.
If a DNN learns lots of visual concepts for classification, then these concepts can be regarded as knowledge points, such as the bird head concept for the bird classification.
If these knowledge points are discriminative enough, then this DNN probably obtains good performance.


(a) Visualization of the information discarding through different layers of VGG-16 on the CUB200-2011 dataset. Input units with darker colors have less information discarding. 
 (b) Comparison of the coherency of different explanation methods. Our method coherently measures how input information is gradually discarded through layers, and enables fair comparisons of knowledge representations between different layers. In comparison, CAM and gradient explanations cannot generate coherent magnitudes of importance values through different layers for fair comparisons. More analysis is presented in Section.
  

The positive correlation between the ratio of foreground knowledge points $\lambda$ and the classification accuracy of DNNs on the CUB200-2011 dataset.}
   

In order to measure the quantity and the quality of knowledge points encoded in the DNN, we consider the signal processing in the forward propagation of a DNN as the process of layer-wise information discarding.
As Figure (a) shows, the DNN gradually discards the information of each input unit in the forward propagation. 
Here, an input unit is referred to as a variable (or a set of variables) in the input sample.
For example, the embedding of each word in the input sentence can be regarded as an input unit for natural language processing.
In the scenario of Figure (a), an input unit is referred to as a pixel (or pixels within a small local region) the input image.
Then, the information of some units (\textit{e.g.} information of pixels in the background) is discarded significantly.
In comparison, information of other input units (\textit{e.g.} information of pixels in the foreground) is less discarded.


In this way, we consider input units without significant information discarding as knowledge points, such as input units of the bird in Figure (a). 
These knowledge points usually encode discriminative information for inference, \textit{e.g.} wings of birds in Figure (a) are discriminative for the fine-grained bird classification.
In comparison, input units with significant information discarding usually do not contain discriminative information for prediction.
Thus, measuring the information discarding of input units enable us to quantify knowledge points.



Besides the quantity of knowledge points, we also measure the quality of knowledge points with the help of annotations of foreground objects.
To this end, we classify all knowledge points into two types, \textit{i.e.} knowledge points related to the task and knowledge points unrelated to the task.
In this way, we can compute the ratio of knowledge points encoded in a DNN that are relevant to the task, as a metric to evaluate the quality of knowledge points. 
A high ratio of relevant knowledge points indicates the feature representation of the DNN is reliable.
Figure shows that DNNs encoding a larger ratio of task-related knowledge points usually achieve better performance
(please see Section for more analysis).


Based on the quantification of knowledge points, we propose the following three hypotheses on reasons why knowledge distillation outperforms traditional learning from scratch. 
Furthermore, we design three types of metrics to verify these hypotheses.



\textbf{Hypothesis 1: Knowledge distillation makes the DNN learn more knowledge points than the DNN learning from scratch.} 
The information-bottleneck theory claimed that a DNN tended to preserve features relevant to the task and neglected those features irrelevant to the task for inference.
We assumed that a teacher network is supposed to achieve superior classification performance, because the teacher network usually has a complex network architecture or is often learned using more training data.
In this scenario, the teacher network is considered to encode more knowledge points related to the task and fewer knowledge points unrelated to the task than the student network.
In this way, knowledge distillation forces the student network to mimic the logic of the teacher network, which ensures the student network models more knowledge points relevant to the task and fewer knowledge points irrelevant to the task than the DNN learning from scratch.


\textbf{Hypothesis 2: Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. In comparison, the DNN learning from scratch tends to encode various knowledge points sequentially through different epochs.} 
It is because knowledge distillation forces the student network to mimic all knowledge points of the teacher network simultaneously.
In comparison, the DNN learning from scratch tends to focus on different knowledge points in different epochs sequentially.


\textbf{Hypothesis 3: Knowledge distillation usually yields more stable optimization directions than learning from scratch.}
The DNN learning from scratch usually keeps trying different knowledge points in early epochs and then discarding unreliable ones in late epochs, rather than model target knowledge points directly.
Thus, the optimization directions of the DNN learning from scratch is inconsistent. 
For convenience, in this paper, the phenomenon of inconsistent optimization directions through different epochs is termed as~\textbf{\textit{``detours''}}\footnote[1]{``Detours'' refer to the phenomenon that a DNN tends to encode various knowledge points in early epochs and discard non-discriminative ones later.}. 


Unlike learning from scratch, knowledge distillation usually forces the student network to mimic the teacher network directly.
The student network straightforwardly encodes target knowledge points without temporarily modeling and discarding other knowledge points.
Thus, the student network is optimized without significant detours.
For a better understanding of Hypothesis 3, let us take the fine-grained bird classification as an example. With the guidance of the teacher network, the student network directly learns discriminative features from heads or tails of birds without significant detours. In comparison, the DNN learning from scratch usually extracts features from the head, belly, tail, and tree-branch in early epochs, and later neglects features from the tree branch. In this case, the optimization direction of the DNN learning from scratch is more unstable.



Note that previous studies of explaining the optimization stability and the generalization power of the DNN were mainly from the perspective of the parameter space.
[1] demonstrated that the flatness of minima of the loss function resulted in good generalization. 
[2] illustrated that the generalization behavior of the network depended on the norm of the weights.
In contrast, this paper explains the efficiency of optimization from the perspective of knowledge representations, \textit{i.e.} analyzing whether or not the DNN encodes different knowledge points simultaneously and without significant detours.



\textbf{Connection to the information-bottleneck theory.}
We roughly consider that the information-bottleneck theory can also be used to explain the change of knowledge points in a DNN. It showed that a DNN usually extracted a few discriminative features for inference, and neglected massive features irrelevant to the inference during the training process.
The information-bottleneck theory measures the entire discrimination power of each sample.
In comparison, our method quantifies the discrimination power of each input unit in a more detailed manner, and measures pixel-wise information discarding through forward propagation.


\textbf{Methods.} 
In order to verify above hypotheses, we design three types of metrics to quantify knowledge points encoded in intermediate layers of a DNN, and analyze how different knowledge points are modeled during the training procedure. 


$\bullet\quad$The first type of metrics measures the quantity and quality of knowledge points.
We consider that a well-trained DNN with superior classification performance is supposed to encode
massive knowledge points, where most knowledge points are discriminative for the classification of target categories.

$\bullet\quad$The second type of metrics measures whether a DNN encodes various knowledge points simultaneously or sequentially, \textit{i.e.} examining whether different knowledge points are learned at similar speeds.

$\bullet\quad$The third metric evaluates whether a DNN is optimized with or without significant detours.
In other words, this metric measures whether or not the DNN directly learns target knowledge points without temporarily modeling and discarding other knowledge points.
To this end, this metric is designed as the overlap between knowledge points encoded by the DNN in early epochs and final knowledge points of the DNN.
If this overlap is large, then we consider this DNN is optimized without significant detours; otherwise, with detours.
It is because a small overlap indicates that 
the DNN first encodes a large number of knowledge points in early epochs, but many of these knowledge points are discarded in later epochs.

In summary, we use these metrics to compare knowledge distillation and learning from scratch, in order to verify Hypotheses 1-3. 

\textbf{Using the annotated knowledge points or not.}
In particular, we should define and quantify knowledge points without any human annotations.
It is because we do not want the analysis of the DNN to be influenced by manual annotations with significant subjective bias, which hurts the trustworthiness of this research.
Besides, the cost of annotating all knowledge points is also unaffordable.
However, previous studies often define visual concepts (knowledge points) by human annotations, and these concepts usually have specific semantic meanings.
For example, Bau manually annotated six types of semantic visual concepts (objects, parts, textures, scenes, materials, and colors) to explain feature representations of DNNs.
In this way, these methods cannot fairly quantify the actual amount of knowledge encoded by a DNN, because most visual concepts are not countable and cannot be defined with human annotations.

In contrast, this paper uses the information discarding of each input unit to define and quantify knowledge points without human annotations.
Such knowledge points are usually referred to as \textit{\textbf{``Dark Matters'' }}.
Compared to traditionally labeled visual concepts, we consider these dark-matter knowledge points can provide a more general and trustworthy way to explain feature representations of DNNs.


\textbf{Scope of explanation.}
A trustworthy explanation of knowledge distillation usually has two requirements.
First, the teacher network is supposed to be well optimized as the student network.
Otherwise, if the teacher network does not converge or is optimized for other tasks, then the teacher network is not qualified for distillation.
Second, knowledge distillation often has two fully different utilities. 
(1) Distilling from high-dimensional features usually forces the student network to mimic all sophisticated feature representations in the teacher network.
(2) Distilling from the low-dimensional network output mainly selectively uses confident training samples for learning, 
with very little information on how the teacher encodes detailed features. 
In this case, the distillation selectively emphasizes the training of simple samples and ignores the training of hard samples\footnote[2]{Confident (simple) samples usually generate salient output signals for knowledge distillation than unconfident (hard) samples.}.
Therefore, in this paper, we mainly explain the first utility of knowledge distillation, 
\textit{i.e.,} forcing the student network to mimic the knowledge of the teacher network.
Such a utility is  mainly exhibited by distilling from high-dimensional intermediate-layer features.


Contributions of this paper are summarized as follows.

1. The quantification of knowledge points encoded in intermediate layers of DNNs can be used as a new perspective to analyze DNNs.

2.  Based on the quantification of knowledge points, we design three types of metrics to explain the mechanism of knowledge distillation.

3. Three hypotheses about knowledge distillation are proposed and verified in different classification applications, including image classification, 3D point cloud classification, binary sentiment classification, and question answering,
which shed new light on the interpretation of knowledge distillation.

A preliminary version of this paper appeared in [1].




\section{Related work}
Although DNNs have shown promises in various applications, they are still regarded as black boxes. Previous studies of interpreting DNNs are roughly summarized as semantic explanations and mathematical analysis of the representation capacity.

$\bullet\quad$\textbf{Semantic explanations for DNNs.} 
An intuitive way to explain DNNs is to visualize the appearance encoded in intermediate layers of DNNs, which may significantly activate a specific neuron of a certain layer. Gradient-based methods measured the importance of intermediate-layer activation units or input units by using gradients of outputs \textit{w.r.t.} inputs. Inversion-based methods  inverted feature maps of convolutional  layers into images. 
Moreover, some studies estimated the pixel-wise or regional attribution/importance/saliency of an input to the network output.

The semantic dissection is also a classical direction of interpreting DNNs. 
Bau manually annotated six types of visual concepts (\textit{objects, parts, scenes, textures, materials} and \textit{colors}), and associated units of DNN feature maps with these concepts. 
Furthermore, the first two concepts could be summarized as shapes, and the last four concepts could be summarized as textures. 
Fong and Vedaldi used a set of filters to represent a single semantic concept, and built up many-to-many projections between concepts and filters. 
TCAV measured the importance of user-defined concepts to classification results.

Learning a DNN with interpretable feature representations in an unsupervised or weakly-supervised manner is another direction of explainable AI. 
InfoGAN and $\beta$-VAE learned interpretable latent representations for generative networks. 
In the capsule network, each capsule encoded different meaningful features. 
Interpretable CNNs were used to make each filter in a high convolutional layer represent a specific object part.  
The BagNet was proposed to classify images based on the occurrences of local image features. 
The ProtoPNet  was introduced to learn prototypical parts.
Shen proposed a method to modify a traditional CNN into an
interpretable compositional CNN.

In summary, previous studies are mainly based on heuristic assumptions to calculate importance/saliency/attention or use massive human-annotated concepts to interpret network features. 
Whereas, in this paper, we explain feature representations from the perspective of knowledge points.


$\bullet\quad$\textbf{Mathematical explanations for the representation capacity of DNNs.} 
Formulating and evaluating the representation capacity of DNNs is an emerging direction of explainable AI. 
The information-bottleneck theory provided a generic metric to quantify the information encoded in DNNs, which can be extended to evaluate the representation capacity of DNNs. 
Zhang discussed the relationship between the parameter number and the generalization capacity of DNNs. 
Weng proposed to use the CLEVER score to measure the robustness of neural networks. 
Fort used the stiffness to diagnose the generalization of a DNN.
The module criticality was proposed to explain the superior generalization performance of some network architectures.

Unlike previous studies, this paper aims to bridge the gap between mathematical explanations and semantic explanations. In other words, we use the information discarding of the input to quantify knowledge points and to explain the discrimination power of the DNN. More specifically, we analyze the quantity and the quality of knowledge points in a DNN, measure whether a DNN encodes various knowledge points sequentially or simultaneously, and evaluate the stability of optimization direction.


$\bullet\quad$\textbf{Knowledge distillation.} 
Knowledge distillation is a popular technique in knowledge transferring, which can be applied to different domains such as adversarial defense, object detection, semantic segmentation, model compression, and improving generalization. 

Although knowledge distillation has achieved success in various applications, there have been very few attempts on explaining how and why it helps the training of the DNN. Hinton demonstrated that learning from ``soft targets'' was easier than learning from ``hard targets".
Furlanello explained the efficiency of knowledge distillation as re-weighting training examples.
From a theoretical perspective, Lopez-Paz related knowledge distillation to learning from privileged information under a noise-free setting.  
Phuong and Lampert explained the success of knowledge distillation from the view of data distribution, optimization bias, and the size of the training set. 
Yuan interpreted knowledge distillation in terms of Label Smoothing Regularization. 
Menon considered that a good teacher modeling the Bayes class-probabilities resulted in the success of knowledge distillation.

However, previous explanations for knowledge distillation were mainly based on 
qualitative statements or theoretically relied on strong assumptions, such as linear models.
In contrast, we interpret knowledge distillation from the perspective of knowledge representations, \textit{i.e.} quantifying, analyzing, and comparing knowledge points encoded in distilled DNNs and knowledge points encoded in DNNs learning from scratch.
Hence, knowledge points provide new insight into the success of knowledge distillation.




\section{Algorithm}
In this paper, we explain the success of knowledge distillation from a new perspective, \textit{i.e.} quantifying knowledge points encoded in the intermediate layers of a DNN for classification.
Unlike previous explanations for knowledge distillation, our method enables people to explain the representation power of a DNN using the quantity and the quality of knowledge points encoded in a DNN, which reflects a more direct and stronger connection between the knowledge and the performance.
To this end, we measure the information discarding of each input unit to define knowledge points in a DNN, based on the information theory.
We propose three hypotheses on the mechanism of knowledge distillation to explain its success.
In order to verify these hypotheses, we further design three types of metrics based on the quantification of knowledge points, which evaluate the representation quality of the DNN.
Note that theoretically, knowledge distillation usually has two fully different utilities.
Distillation from high-dimensional intermediate-layer features usually exhibits the first type of utilities,~\textit{i.e.,} forcing the student network to mimic knowledge points of the teacher network.
Whereas, distilling from relatively low-dimensional network output often exhibits the second type of utilities,~\textit{i.e.,} selecting confident samples for learning and ignoring  unconfident samples.
In this paper, we mainly explain the first utility of knowledge distillation, which is mainly exhibited by distilling from high-dimensional intermediate-layer features.


\subsection{Quantifying Information Discarding}
Before defining and quantifying knowledge points encoded in DNNs, we first introduce how to measure the pixel-wise information discarding of the input sample in this section.

According to information-bottleneck theory, we consider the signal processing of a forward propagation as the layer-wise discarding of input information.
In low layers, most input information is used to compute features.
Whereas, in high layers, information in input units unrelated to the inference is gradually discarded, and only related pixel-wise information is maintained in the computation of network features.
In this way, we consider features of the highest layer mainly encode the information, which is highly relevant to the inference.

Thus, we propose methods to quantify the input information encoded in a specific intermediate layer of a DNN, \textit{i.e.} measuring how much input information is discarded when the DNN extracts the feature of this layer.
 To this end, the information discarding of each input unit is formulated as the entropy, given a feature of a certain network layer.
 
Specifically, given a trained DNN for classification and an object instance $x\in{R^{n}}$ with $n$ input units, let $f^{*}=f(x)$ denote the feature of a network intermediate layer, 
and let $y^{*}$ denote the network prediction~\textit{w.r.t.} $x$.
The input unit is referred to as a variable (or a set of variabels) in the input sample.
For example, each pixel (or pixels within a small local region) of an input image can be taken as an input unit, 
and the embedding of each word in an input sentence also can be regarded as an input unit.


In our previous works, 
we consider that the DNN satisfies the Lipschitz constraint
$\parallel{y'-y^{*}}\parallel \le \kappa \parallel{f(x')-f^{*}}\parallel^{2}$, where $\kappa$ is the Lipschitz constant, and $y'$ corresponds to the network prediction of the sample $x'$.
The  Lipschitz constant $\kappa$ can be computed as the maximum norm of the gradient within a small range of features,~\textit{i.e.,}
{\small$\kappa = \max_x \parallel{\nabla f(x)}\parallel$}.
In fact, for any continuous function without a singular point, there often exists a Lipschitz constant for this function.
Besides, many previous studies assumed that a DNN has such a specific Lipschitz constant.
This indicates that 
If we add a small perturbation to the intermediate-layer feature, then the change of the DNN's output is also limited,~\textit{i.e.,} $\parallel{y'-y^{*}}\parallel \le \delta f$.
In other words,
the DNN usually represents a specific object instance using a very limited range of features $\small{ \parallel{f(x')-f^{*}}\parallel ^{2}\le \tau}$, where $\tau$ is a  positive scalar and $f(x')$ denotes the feature in the limited range.
In other words, all features in $\small{\{f(x')\big{|} \parallel{f(x')-f^{*}}\parallel ^{2}\le \tau\}}$ represent the same object instance, 
\textit{i.e.}, $\small{\parallel{y'-y^{*}}\parallel \le \kappa \cdot \tau}$.


However, it is very difficult to determine the explicit low-dimensional manifold of features \textit{w.r.t.} the input $x$.
As an expediency, we add perturbations $\Delta x$ to the input sample $x$ to approximate the manifold of the feature, \textit{i.e.} generating samples 
$x'= x+\Delta x$, subject to
$\small{ \parallel{f(x')-f^{*}}\parallel ^{2}\le \tau}$.
In this way, the entropy $H(X')$ measures the uncertainty of the input when the feature represents the same object instance, 
$\small{\parallel{y'-y^{*}}\parallel \le \kappa \cdot \tau}$, as mentioned above.
In other words, $H(X')$ quantifies how much input information can be discarded without affecting the inference of the object.
$X'$ denotes a set of inputs corresponding to the concept of a specific object instance. 
It is assumed that $\Delta x$ is an \textit{i.i.d.} Gaussian noise, thereby $x'= x+\Delta x \sim \mathcal{N}(x,\Sigma(\boldsymbol\sigma) = diag(\sigma_{1}^{2},\dots, \sigma_{n}^{2}))$.
Here, $\sigma_{i}$ indicates the variance of the perturbation \textit{w.r.t.} the $i$-th input unit.
The assumption of the Gaussian distribution ensures that the entropy $H(X') $ of the input can be decomposed into pixel-level entropies $\{H_{i}\}$.
\begin{equation}\label{2}
\small{H(X') = \sum_{i=1}^{n} H_{i},}
\end{equation}
where $H_{i} = \log\sigma_{i} +  \frac{1}{2} \log(2\pi{e})$ measures the pixel-wise information discarding. 
A large value of $H_{i}$ usually indicates that the information of the $i$-th unit is significantly discarded during the forward propagation.
For example, as Figure~\ref{fig:layer}(a) shows, information encoded in background pixels is significantly discarded for the fine-grained bird classification.



Thus, we learn the optimal $\Sigma(\boldsymbol\sigma) = diag(\sigma_{1}^{2},\dots, \sigma_{n}^{2})$ via the maximum-entropy principle to compute the pixel-wise information discarding $H_{i}= \log\sigma_{i} +  \frac{1}{2} \log(2\pi{e})$.
The objective function is formulated in Equation, which maximizes $H(X')$ subject to constraining features within the scope of a specific object instance $\small{\parallel{f(x')-f^{*}}\parallel ^{2}\le \tau}$.
\textit{I.e.,} we enumerate all perturbation directions in the input sample $x$ within a small variance of the feature $f^{*}$, in order to approximate the low-dimensional manifold of $f(x')$. 
We use the Lagrange multiplier to approximate Equation as the following loss.
Considering Equation is intractable, we use $x'=x+{\boldsymbol\sigma}\circ{\boldsymbol\delta}, \delta\sim\mathcal{N}(0,I)$ to simplify the computation of $\text{Loss}({\boldsymbol\sigma})$, where {\small$\circ$} denotes the element-wise multiplication.
{\small${\boldsymbol\sigma}=[\sigma_1,\ldots,\sigma_{n}]^{\top}$} represents the range that the input sample can change.
In this way, $\text{Loss}({\boldsymbol\sigma})$ in Equation is tractable, and we can learn $\boldsymbol\sigma$ via gradient descent.
{\small $\delta_f^2 = \lim_{\tau\rightarrow0^{+}}\mathbb{E}_{x'\sim\mathcal{N}(x,\tau{^2} I )}\left[\Vert f(x')-f^{*}\Vert^2\right]$} denotes the inherent variance of intermediate-layer features subject to small input noises with a fixed magnitude $\tau$. $\delta_f^2$ is used for normalization, and a positive scalar $\alpha$ is used to balance the two loss term.




\subsection{Quantification of knowledge points}
\textbf{Hypothesis 1}: Knowledge distillation makes the DNN encode more knowledge points than learning from scratch.




The basic idea is to measure the quantity and quality of knowledge points encoded in intermediate layers of a DNN.



Visualization of knowledge points. The dark color indicates the low entropy value ${H_{i}}$. Image regions with low pixel-wise entropies ${\{H_{i}\}}$ are considered as knowledge points. In real implementation, to improve the stability and efficiency of the computation, we divide the image into $16\times16$ grids, and each grid is taken as a ``pixel" to compute the entropy $H_{i}$.





$\bullet\quad$\textbf{The quantity of knowledge points.}
In this paper, we use the pixel-wise information discarding of each input unit to define and quantify knowledge points.
Given a trained DNN and an input sample $x \in X$, let us focus on the pixel-wise information discarding ${H_{i}}$ \textit{w.r.t.} the feature of a certain network layer $f^{*}=f(x)$.
$X$ represents a set of input samples.

According to Equation~\eqref{2}, a low pixel-wise entropy $H_{i}$ represents the information of this input unit is less discarded.
In other words, the DNN tends to use these input units with low entropies to compute the feature $f^{*}$ and make the inference.
Thus, a knowledge point is defined as an input unit with a low pixel-wise entropy $H_{i}$, which encodes discriminative information for prediction.
For example, bird heads in Figure~\ref{fig1} are referred to as knowledge points, which are useful for the fine-grained bird classification.

To this end, we use the average entropy $\overline{H}$ of all background units $\Lambda_{\textrm{bg}}$ as a baseline to determine knowledge points, \textit{i.e.} $\overline{H}=\mathbb{E}_{i \in \Lambda_{\textrm{bg}}}[H_{i}]$.
It is because information encoded in background units is usually supposed to be significantly discarded and irrelevant to the inference.
If the entropy of a unit is significantly lower than the baseline entropy $\overline{H} - H_{i} > b$, then this input unit can be considered as a valid knowledge point.
Here, $b$ is a threshold to determine the knowledge points, which is introduced in Section~\ref{Implementation Details}.
In this way, we can quantify the number of knowledge points in the DNN.

$\bullet\quad$\textbf{The quality of knowledge points.}
Besides the quantity of knowledge points, we also consider the quality of knowledge points.
Generally speaking, information encoded in foreground units is usually supposed to be crucial to the inference.
In comparison, information encoded in background units is often supposed to have negligible effects on the prediction.
Therefore, we design a metric $\lambda$ to evaluate the quality of knowledge points by examining whether or not most knowledge points are localized in the foreground.
$N_{\textrm{point}}^{\textrm{bg}}(x)$ and $N_{\textrm{point}}^{\textrm{fg}}(x)$ denote the number of knowledge points encoded in the background and the foreground, respectively.
$\Lambda_{\textrm{bg}}$ and $\Lambda_{\textrm{fg}}$ are sets of input units in the background and the foreground \textit{w.r.t.} the input sample $x$, respectively.
$\mathbbm{1}(\cdot)$ refers to the indicator function. If the condition inside is valid, then $\mathbbm{1}(\cdot)$ returns $1$; otherwise, returns $0$.
A large value $\lambda$ represents the feature representation of the DNN is reliable; otherwise, unreliable.

Thus, knowledge points provide a new way to explain the mechanism of knowledge distillation, \textit{i.e.} checking whether or not knowledge distillation makes the DNN encode massive knowledge points, and whether or not most knowledge points are precisely localized in the foreground.




Comparisons of different explanation methods in terms of the coherency. The coherency of the entropy-based method enables fair layer-wise comparisons within a network, and fair comparisons between different networks.




\textbf{Coherency and generality}.
As discussed in [1], a trustworthy explanation method to evaluate feature representations of the DNN should satisfy criteria of the coherency and generality.
From this perspective, we analyze the trustworthiness of knowledge points.

The \textbf{coherency} indicates the explanation method should reflect the essence of the encoded knowledge representations in DNNs, which are invariant to network settings.
In this paper, we use pixel-wise information discarding to define knowledge points without strong assumptions of feature representations, or network architectures.
In this way, knowledge points yield a coherent evaluation of feature representations.
However, most existing explanation methods in Table usually fail to meet this criterion due to their biased assumptions. 
For example, the CAM and gradient explanations do not generate coherent explanations, because the gradient map $\frac{\partial Loss}{\partial f}$ is usually not coherent through different layers.

To this end, we compare our method with  the CAM and the gradient explanations.
Theoretically, we can easily construct two DNNs representing exactly the same knowledge but with different magnitudes of gradients, as follows.
A VGG-16 model was learned using the CUB200-2011 dataset for fine-grained bird classification.
Given this pre-trained DNN, we slightly revised the magnitude of parameters in every pair of neighboring convolutional layers {\small$y=x\otimes w+b$} to examine the coherency.
For the {\small$L$}-th and {\small$(L+1)$}-th layers, parameters were revised as {\small$w^{(L)}\leftarrow 4w^{(L)}$}, {\small$w^{(L+1)}\leftarrow w^{(L+1)}/4$}, {\small$b^{(L)}\leftarrow 4b^{(L)}$}, {\small$b^{(L+1)}\leftarrow b^{(L+1)}/4$}.
Such revisions did not change knowledge representations or the network output, but changed the gradient magnitude.

As Figure (b) shows, magnitudes of the CAM and the gradient explanation methods are sensitive to the magnitude of parameters. In comparison, our method is not affected by the magnitude of parameters, which demonstrates the coherency. Thus, the coherency of our method enables fair layer-wise comparisons within a DNN, and fair comparisons between different DNNs.

The \textbf{generality} means that the explanation method should have strong connections to existing mathematical theories.
To this end, we quantify knowledge points using the entropy of the input sample.
The entropy is a generic tool with strong connections to various theories, \textit{e.g.} the information-bottleneck theory.
As a result, the generality of knowledge points enables us to fairly compare feature representations between different DNNs.
Note that calculating knowledge points requires the annotation of the foreground, but this requirement does not hurt the coherency and the generality of knowledge points.




\subsection{Learning simultaneously or sequentially}
\textbf{Hypothesis 2}: Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. Whereas, the DNN learning from scratch tends to encode various knowledge points sequentially in different epochs.



Procedure of learning foreground knowledge points \textit{w.r.t.} weight distances. According to information-bottleneck theory, a DNN tends to learn various knowledge points in early epochs and then discard knowledge points irrelevant to the task later. Strictly speaking, a DNN learns new knowledge points and discards old ones during entire the learning process. The epoch $\hat{m}_{x}$ encodes the richest foreground knowledge points.}





This hypothesis can be understood as follows.
Knowledge distillation forces the student network to mimic all knowledge points of the teacher network simultaneously.
In comparison, the DNN learning from scratch is more likely to learn different knowledge points in different epochs.
A DNN learning from scratch may encode knowledge points of common, simple, and elementary features in early epochs.
For example, in the scenario of fine-grained bird classification, the sky is a typical and simple feature to learn.
Whereas, knowledge points representing complex features may be encoded in later epochs by the DNN learning from scratch.
For example, in the scenario of fine-grained bird classification, the subtle difference between two similar bird species is difficult to learn.
In this way, the DNN learning from scratch tends to encode different knowledge points in a sequential manner, rather than simultaneously.

\textbf{Metrics.}
In order to verify Hypothesis 2, we design two metrics, which examines whether or not 
different knowledge points are learned within similar epochs, \textit{i.e.} whether or not learning different knowledge points simultaneously.

Specifically, given a set of training samples $X$, let $M$ denote the total epochs to train a DNN.
For each specific sample $x\in X$, foreground knowledge points learned by DNNs after $j$ epochs are represented as 
$N_{j}^{\textrm{fg}}(x)$, where $j \in \{1,2,\cdots,M\}$.

In this way, whether or not a DNN learns different knowledge points simultaneously can be measured from the following two aspects.
(1) Whether or not the number of foreground knowledge points $N_{j}^{\textrm{fg}}(x)$ increases fast along with the epoch number.
(2) Whether or not $N_{j}^{\textrm{fg}}(x)$~\textit{w.r.t.} different samples increase simultaneously.
In other words, the first aspect measures whether or not the DNN learns various knowledge points of a specific input sample quickly, and the second aspect evaluates whether a DNN learns knowledge points of different samples at similar speeds.

To this end, as Figure shows, we consider the epoch $\hat{m}$ that a DNN obtains richest foreground knowledge points to measure the learning speeds, 
\textit{i.e.} $\hat{m}_{x} = \arg\max_{k} N_{k}^{\textrm{fg}}(x)$.
We use metrics $D_{\textrm{mean}}$ and $D_{\textrm{var}}$ based on the \textit{``weight distance'' } $\sum_{k=1}^{{m}} \frac{\|{w_{k}-w_{k-1}}\|}{\|{w_{0}}\|}$ to check whether a DNN learns knowledge points simultaneously or not.
$w_{0}$ and $w_{k}$ denote initial parameters and parameters learned after the $k$-th epoch, respectively.
The metric $D_{\textrm{mean}}$ represents the average weight distance that the DNN obtains the richest foreground knowledge points, and
the metric $D_{\textrm{var}}$ describes the variation of the weight distance \textit{w.r.t.} different input samples.
These two metrics are defined as follows.
Here, we use the weight distance  to evaluate the learning effect at each epoch, rather than use the epoch number.
It is because the weight distance better quantifies the total path of updating the parameter $w_{k}$ at each epoch $k$ than the epoch number.
In other words, the weight distance can better measure the dynamic learning process of the DNN.
In this way, $D_{\textrm{mean}}$ measures whether a DNN learns knowledge points quickly, and $D_{\textrm{var}}$ evaluates whether a DNN learns knowledge points of different input samples at similar speeds.
Thus, small values of $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ reflect that the DNN learns various knowledge points quickly and simultaneously.







\subsection {Learning with Less Detours}
\textbf{Hypothesis 3}: Knowledge distillation usually yields more stable optimization directions than learning from scratch.



Detours of learning knowledge points. We visualize sets of foreground knowledge points learned after different epochs. The green box indicates the union of knowledge points learned during all epochs. The $(1-\rho)$ value denotes the ratio of knowledge points that are discarded during the learning process to the union set of all learned knowledge points. A larger $\rho$ value indicates DNN is optimized with fewer detours.
    


This hypothesis can be understood as follows.
According to the information-bottleneck theory, the DNN learning from scratch usually tries to model various knowledge points in early epochs and then discards those unrelated to the inference in late epochs.
It means that the DNN learning from scratch cannot directly encode target knowledge points for inference.
Thus, the optimization direction of this DNN is inconsistent and unstable in early and late epochs, \textit{i.e.} with significant detours.
Unlike learning from scratch, knowledge distillation forces the student network to directly mimic the well-trained teacher network.
With the guidance of the teacher network, knowledge distillation makes the student network straightforwardly model target knowledge points without temporarily modeling and discarding other knowledge points.
Thus, the DNN learning via knowledge distillation tends to be optimized in a stable direction, \textit{i.e.} without significant detours.


\textbf{Metric.}
In order to verify Hypothesis 3, we design a metric to evaluate whether a DNN is optimized in a stable and consistent direction or not.
Let $S_{j}(x)=\{i\in x|\overline{H} - H_{i} > b\}$ denote the set of foreground knowledge points in the input sample $I$ encoded by the DNN learned after the $j$-th epoch, where $j\in\{1,2,\cdots,M\}$.
Each knowledge point $a \in{S_{j}(x)}$ is referred to as a specific unit $i$ on the foreground of the input sample $I$, which satisfies $\overline{H} - H_{i} > b$. 
Then, we use the metric $\rho$ to measure the stability of optimization directions.
$\rho$ represents the ratio of finally encoded knowledge points to all temporarily tried knowledge points in intermediate epochs, where $|\cdot|$ denotes the cardinality of the set.
More specifically, the numerator of Equation reflects the number of foreground knowledge points, which have been chosen ultimately for inference.
For example, knowledge points in the black box of Figure are encoded as final knowledge points for the fine-grained bird classification.
The denominator represents the number of all knowledge points temporarily learned during the entire training process, which is shown as the green box in Figure.
Moreover, $(\bigcup_{j=1}^{M} S_{j}(x)\setminus{S_{M}(x))}$ indicates a set of knowledge points, which have been tried, but finally are discarded by the DNN. 
The set of those discarded knowledge points is shown as the brown box in Figure.
Thus, a high value of $\rho$ indicates that the DNN is optimized without significant detours and more stably; otherwise, with significant detours.



\section{Experiment}
In this section, we conducted comparative experiments on image classification, 3D point cloud classification, and natural language processing (NLP) tasks. These experiments verified the proposed hypotheses.




\subsection{Implementation Details}
Given a teacher network, we distilled knowledge from the teacher network to the student network.
In order to remove the effects of network architectures, the student network had the same architecture as the teacher network.
Meanwhile, for fair comparisons, the DNN learning from scratch was also required to have the same architecture as the teacher network.
For convenience,  we named the DNN learning from scratch the \textbf{baseline network} in the following manuscript. 



Additionally, we conducted experiments to check whether the size of the teacher network hurt the verification of three hypotheses.
Tables show when the student network distilled from a larger teacher network, Hypotheses 1-3 were still verified.
This phenomenon indicates that the change of teacher network size did not hurt the verification of our conclusions.
To simplify the story, we set student networks to have the same architectures as teacher networks in the following experiments.



Comparisons between the student network and the baseline network (B) for the image classification on the CUB200-2011 dataset, where student network distilled from $\textrm{FC}_{1}$ layer of a larger teacher network.




Comparisons between the student network (S) and the baseline network (B) for image classification on the CUB200-2011 dataset, respectively. 
Metrics were evaluated at the $\textrm{FC}_{1}$ layer under different settings of the grid size and different settings of the threshold $b$. Experimental results verified Hypotheses 1-3.





\textbf{Datasets \& DNNs.} 
\textit{For the image classification task}, we conducted experiments based on AlexNet, VGG-11, VGG-16, VGG-19, ResNet-50, ResNet-101, and ResNet-152. 
We trained these DNNs based on the ILSVRC-2013 DET dataset, the CUB200-2011 dataset, and the Pascal VOC 2012 dataset for object classification, respectively. 
Considering the high computational burden of training on the entire ILSVRC-2013 DET dataset, we conducted the classification of terrestrial mammal categories for comparative experiments.
Note that all teacher networks were pre-trained on the ImageNet dataset, and then fine-tuned using the aforementioned dataset. 
In comparison, all baseline networks were learned from scratch. 
Moreover, data augmentation was applied to 
both the student network and the baseline network, when DNNs were learned using the ILSVRC-2013 DET dataset or the Pascal VOC 2012 dataset.


We used object images cropped by object bounding boxes to train the aforementioned DNNs on each above dataset, respectively.
In particular, to achieve stable results, images in the Pascal VOC 2012 dataset were cropped by using $1.2 \,{width} \times 1.2 \,{height}$ of the original object bounding box. 
For the ILSVRC-2013 DET dataset, we cropped each image by using $1.5 \,{width} \times 1.5 \,{height}$ of the original object bounding box. 
It is because there existed no ground-truth annotations of object segmentation for the ILSVRC-2013 DET dataset.
We used the object bounding box to separate foreground regions and background regions of images in the ILSVRC-2013 DET dataset.
In this way, pixels within the object bounding box were regarded as the foreground~$\Lambda_{\textrm{fg}}$, and pixels outside the object bounding box were referred to as the background~$\Lambda_{\textrm{bg}}$.

\textit{For natural language processing}, we fine-tuned a pre-trained BERT model using the SQuAD dataset as the teacher network towards question answering.
Besides, we also fine-tuned another pre-trained BERT model on the SST-2 dataset as the teacher network for binary sentiment classification.
Baseline networks and student networks were just trained using samples in the SST-2 dataset or the SQuAD dataset.
Moreover, for both the SQuAD dataset and the SST-2 dataset, we annotated input units irrelevant to the prediction as the background~$\Lambda_{\textrm{bg}}$, according to the human cognition.
We annotated units relevant to the inference as the foreground~$\Lambda_{\textrm{fg}}$.
For example, words related to answers were labeled as foregrounds in the SQuAD dataset. Words containing sentiments were annotated as foregrounds in the SST-2 dataset.

\textit{For 3D point cloud classification task}, we conducted comparative experiments on the PointNet, DGCNN, PointConv, and PointNet++ models.
Considering most widely used benchmark datasets for point cloud classification only contained foreground objects, we constructed a new dataset containing both foreground objects and background objects based on the ModelNet40 dataset, as follows.
For each sample (\textit{i.e.} the foreground object) in the ModelNet40 dataset, 
we first randomly sampled five point clouds, whose labels are different from the foreground object. 
Then, we randomly selected $500$ points from the sampled five point clouds, and attached these points to the foreground object as background points.
Moreover, the teacher network was trained using all training data in this generated dataset for classification.
In comparison, we only randomly sampled $10\%$ training data in this generated dataset to learn baseline networks and student networks, respectively.
Thus, the teacher network was ensured to encode better knowledge representations.



\textbf{Distillation.} 
Given a well-trained teacher network and an input sample $x$, we selected a convolutional layer or a fully-connected (FC) layer $l$ as the target layer to perform knowledge distillation.
We used the distillation loss $\|f_{T}(x)-f_{S}(x)\|^{2}$ to force the student network to mimic the feature of the teacher network.
Here, $f_{T}(x)$ denoted the feature of $l$-th layer in the teacher network, and $f_{S}(x)$ indicated the feature of $l$-th layer in its corresponding student network.


In order to simplify the story, we used the distillation loss to learn the student network, rather than the classification loss.
Given the distilled features, we further learned parameters above the target layer $l$ merely using the classification loss.
In this way, we could ensure that all knowledge points of student network were exclusively learned via distillation.
Otherwise, if we trained the student network using both the distillation loss and the classification loss, then it would be hard to distinguish whether the classification loss or the distillation loss was responsible for the learning of each knowledge point. 



Moreover, we employed two schemes of knowledge distillation in this paper,~\textit{i.e.} learning from intermediate-layer features and learning from network output.
Specifically, 
we distilled features in the top convolutional layer ($\textrm{Conv}$) or in each of three FC layers (namely $\textrm{FC}_{1}$, $\textrm{FC}_{2}$ and $\textrm{FC}_{3}$) of the teacher network to train the student network, respectively.
In this way, knowledge distillation from the $\textrm{FC}_{3}$ layer corresponded to the scheme of learning from output, and distillation from other layers corresponded to the scheme of learning from intermediate-layer features.
In spite of these two schemes, we mainly explained knowledge distillation from intermediate-layer features 
that forced the student network to mimic the knowledge of the teacher network as discussed before.



\textbf{The layer used to quantify knowledge points.} 
For each pair of the student network and the baseline network, we measured knowledge points on the top convolutional layer and all FC layers.

Particularly, for DNNs learned on the ILSVRC-2013 DET dataset and the Pascal VOC 2012 dataset, we quantified knowledge points only on $\textrm{FC}_{1}$ and $\textrm{FC}_{2}$ layers,
because the dimension of features in the output layer $\textrm{FC}_{3}$ was much fewer than that of intermediate-layer features in the $\textrm{FC}_{1}$ and $ \textrm{FC}_{2}$ layers.
Similarly, for DNNs trained on the ModelNet40 dataset, we also used the $\textrm{FC}_{1}$ and $ \textrm{FC}_{2}$ layers to quantify knowledge points.
For the BERT model, we measured knowledge points on its last hidden layer.
Considering ResNets usually only had one FC layer, to obtain rich knowledge representations, we added two $\textrm{Conv}$ layers and two FC layers before the last FC layer.
In this way, we quantified knowledge points on these three FC layers.




\textbf{Hyper-parameter settings.}
We used the SGD optimizer, and set the batch size as 64 to train DNNs. 
We set grid size to $16 \times 16$, and settings of the threshold $b$ was as follows.
For DNNs towards image classification, $b$ was set to $0.2$, except that we set $b$ to $0.25$ for AlexNet.
For BERT towards NLP tasks, $b$ was set to $0.2$.
For DNNs towards 3D point cloud classification,  $b$ was set to $0.25$, besides that $b$ was set to $0.5$ for PointNet.


Additionally, we also tested the influence of the grid size and the threshold $b$ on the verification of the three hypotheses.
To this end, we conducted experiments with different settings of the grid size and different settings of the threshold $b$.
Table~\ref{tab:grid_size_b} shows that Hypotheses 1-3 were still validated, when knowledge points were calculated under different different settings of the grid size and different settings of the threshold $b$.



Comparisons of knowledge points encoded in the teacher network (T), the student network (S) and the baseline network (B) for image classification. The teacher network encoded more foreground knowledge points $N_{\textrm{point}}^{\textrm{fg}}$ and obtained a larger ratio $\lambda$ than the student network. Meanwhile, the student network had larger values of $N_{\textrm{point}}^{\textrm{fg}}$ and $\lambda$ than  baseline network.


Visualization of knowledge points encoded in the $ \textrm{FC}_{1}$ layer of VGG-11. Generally, the student network  had a larger $N_{\textrm{point}}^{\textrm{fg}}$ value and a smaller $N_{\textrm{point}}^{\textrm{bg}}$ value than the baseline network.



Comparisons between the student network (S) and the baseline network (B) for image classification. In general, the student network had larger values of $N_{\textrm{point}}^{\textrm{fg}}$, $\lambda$, $\rho$, and smaller values of $N_{\textrm{point}}^{\textrm{bg}}$, $D_{\textrm{mean}}$, $D_{\textrm{std}}$ than the baseline network, which verified Hypotheses 1-3.



Comparisons between the student network (S) and the baseline network (B) for the question answering task and the sentiment classification task, respectively. Metrics were evaluated at the last hidden layer of the BERT model, which verified Hypotheses 1-3.



Comparisons between the student network (S) and the baseline network (B) for the classification of 3D point clouds. In general, Hypotheses 1-3 were verified.


Comparisons between the student network (S) and the baseline network (B) for image classification on the MSCOCO dataset. Metrics were evaluated at $\textrm{FC}_{3}$ layer.




\subsection{Verification of Hypothesis 1}
According to Hypothesis 1, a well-trained teacher network was supposed to encode more foreground knowledge points than the student network and the baseline network. 
Consequently, a distilled student network was supposed to model more foreground knowledge points than the baseline network.
It is because the teacher network was usually trained using a large number of training data, and achieved superior performance to the baseline network.
In this way, this well-trained teacher network was supposed to encode more foreground knowledge points than the baseline network. 
Knowledge distillation forced the student network to mimic the teacher network.
Hence, the student network was supposed to model more foreground knowledge points than baseline network.

$\bullet\quad$\textbf{Quantification of knowledge points in the teacher network, the student network and the baseline network.}
Here, we compared knowledge points encoded in the teacher network, the student network, and the baseline network, and verified the above hypothesis.
We learned a VGG-16 model from scratch as the teacher network using the ILSVRC-2013 DET dataset or the CUB200-2011 dataset towards image classification. 
Data augmentation was used to boost the performance of the teacher network.
Table compares the number of foreground knowledge points $N_{\textrm{point}}^{\textrm{fg}}$ learned by the teacher network, the baseline network, and the student network.
For fair comparisons, the student network had the same architecture as the teacher network and the baseline network according to Section.

Table shows that the teacher network usually encoded more foreground knowledge points $N_{\textrm{point}}^{\textrm{fg}}$ and a higher ratio $\lambda$ than the student network.
Meanwhile, the student network often obtained larger values of $N_{\textrm{point}}^{\textrm{fg}}$ and $\lambda$ than the baseline network.
In this way, the above hypothesis was verified.
There was an exception when $N_{\textrm{point}}^{\textrm{fg}}$ was measured at the $\textrm{FC}_{2}$ layer of the VGG-16 model on the ILSVRC-2013 DET dataset.
The teacher network encoded fewer foreground knowledge points than the student network, because this teacher network had a larger average background entropy value $\overline{H}$  than the student network.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


$\bullet\quad$\textbf{Comparing metrics of $N_{\textrm{point}}^{\textrm{fg}}$, $N_{\textrm{point}}^{\textrm{bg}}$ and $\lambda$ to verify Hypothesis 1.}
Unlike the previous subsection learning the teacher network from scratch, in this subsection, we compared $N_{\textrm{point}}^{\textrm{fg}}$, $N_{\textrm{point}}^{\textrm{bg}}$ and $\lambda$ between the student network and the baseline network when using a more sophisticatedly trained teacher network.
In other words, this teacher network was pre-trained on the ImageNet dataset, and then fine-tuned using the ILSVRC-2013 DET dataset, the CUB200-2011 dataset, or the Pascal VOC 2012 dataset. 
This is a more common case in real applications.


Based on the information discarding $\{H_{i}\}$, we visualized image regions in the foreground that corresponded to foreground knowledge points, as well as image regions in the background that corresponded to background knowledge points in Figure~\ref{fig4}, where these knowledge points were measured at the $\textrm{FC}_{1}$ layer of the VGG-11 model.
In this scenario, Hypothesis 1 was also successfully verified.
Moreover, for tasks of image classification, natural language processing, and 3D point cloud classification, 
Table validated Hypothesis 1.
Very few student networks in Table encoded more background knowledge points $N_{\textrm{point}}^{\textrm{bg}}$ than the baseline network. 
It is because teacher networks in this subsection were either pre-trained or trained using more samples, which encoded knowledge points far more than necessary.
In this way, student networks distilled from these well-trained teacher network learned more unnecessary knowledge for inference, thereby leading to a larger $N_{\textrm{point}}^{\textrm{bg}}$ value than the baseline network.



Note that as discussed in Section, knowledge distillation had two different utilities.
The utility of distilling from the low-dimensional network output was mainly to select confident training samples for learning, with very little information on how the teacher network encoded detailed features.
Whereas, the utility of distilling from  high-dimensional intermediate-layer features was mainly to force the student network to mimic knowledge points of the teacher network.
Hence, in this paper, we mainly explained knowledge distillation from high-dimensional intermediate-layer features.


To this end, in Table, we mainly focused on distillation from intermediate-layer features.
Nevertheless, we conducted another experiment to verify that the utility of distilling from relatively low-dimensional network output was to select confident samples and ignore unconfident samples.
Specifically, we distilled the student network from the $10-$dimensional final output of the teacher network for the classification of the top-10 largest categories in the MSCOCO dataset.
Results in Table illustrated the difference between the two utilities of knowledge distillation, to some extent.
For distilling from the 200-dimensional output for the classification on the CUB200-2011 dataset in Table, the Hypothesis 1 was verified, because the network output with $200$ dimensions encoded relatively rich information to force the student network to mimic knowledge points of the teacher network, which reflected the first utility of knowledge distillation.
Whereas, when the network output had very few dimensions, such as 10-category classification on the MSCOCO dataset in Table,  the student network tended to encode both fewer foreground knowledge points and fewer background knowledge points than learning from scratch.
This phenomenon verified the second utility of sample selection.




Additionally, unlike $\textrm{FC}$ layers, convolutional layers were usually not sufficiently fine-tuned due to their depth, when the teacher networks were first pre-trained on the ImageNet dataset for 1000-category classification, and then were fine-tuned using the CUB200-2011 dataset or the Pascal VOC 2012  dataset.
In this scenario, convolutional layers of the teacher network might encode some noisy features, such as features pre-trained for massive unrelated ImageNet categories.
This might violate the first requirement for the knowledge distillation~\textit{i.e.,} the teacher network was supposed to be well optimized for the same task as the student network.
Hence, in order to analyze the convolutional layer in a stricter manner, we conducted another experiment.
Specifically, we fine-tuned the teacher network on the Tiny ImageNet dataset, which was much larger and already had contained sufficient
training images to ensure that features in high convolutional layers were sophisticatedly fine-tuned. 
Table shows that most hypotheses were verified, except that the student network might encode more background knowledge points than the baseline network.
It was because the teacher network encoded significantly more foreground knowledge points in convolutional layers than the baseline network. 
As a cost, the teacher network also encoded a bit more background knowledge points than the baseline network. 
Therefore, the student network encoded much more foreground knowledge points than the baseline network ($3.9$ more foreground knowledge points on average), but just increased background knowledge points by $1.1$.
Nevertheless, the student network still exhibited a larger ratio of foreground knowledge points than the baseline network.
We considered this phenomenon was still reasonable, which had been explained above.



\textbf{Correlation between the quality of knowledge points and classification performance.}
We conducted experiments to check whether the DNN encoding a larger ratio of foreground knowledge points $\lambda$ usually achieved better classification performance, which has been discussed in Section.
To this end, we used the aforementioned student network to describe how the ratio $\lambda$ changes in different epochs of the training process, which was distilled from $\textrm{FC}_1$ layer of the teacher network on the CUB200-2011 dataset for object classification.
Figure shows that DNNs with a larger ratio of task-related knowledge points often exhibited better performance.




Comparison of {\small{$N_{\textrm{point}}^{\textrm{fg}}$}}, {\small{$N_{\textrm{point}}^{\textrm{bg}}$}} and all knowledge points {\small{$N_{\textrm{point}}^{\textrm{all}}= N_{\textrm{point}}^{\textrm{fg}}+ N_{\textrm{point}}^{\textrm{bg}}$}} between fine-tuning a pre-trained VGG-16 network and learning a VGG-16 network from scratch on the Tiny-ImageNet dataset. Metrics were measured at the highest convolutional layer. The fine-tuning process made the DNN encode new foreground knowledge points more quickly and be optimized with fewer detours than learning from scratch.




Comparisons between the student network (S) and the baseline network (B) for image classification on the Tiny-ImageNet dataset. Metrics were evaluated at $\textrm{Conv}$ layer, where Hypotheses 1-3 were verified, to some extent.




\subsection{Verification of Hypothesis 2}
For Hypothesis 2, we assumed that knowledge distillation made the student network learn different knowledge points simultaneously. To this end, we used metrics $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ to verify this hypothesis.

For image classification,
Table \ref{tab:image class} shows that values of $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ were usually smaller than those of the baseline network, which verified Hypothesis 2.
Notice that there exists a very few failure cases. For example, the $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ were measured at the $\textrm{FC}_{1}$ layer of  AlexNet or at the $\textrm{Conv}$ layer of VGG-11. 
It is because both the AlexNet model and the VGG-11 model had relatively shallow network architectures.
When learning from raw data, DNNs with shallow architectures would be easier to learn more knowledge points with less overfitting.


For NLP tasks (question answering and sentiment classification) and the classification of 3D point clouds, 
Table show that the student network had smaller values of $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ than the baseline network, respectively, which successfully verified Hypothesis 2.






\subsection{Verification of Hypothesis 3}
Hypothesis 3 assumed that knowledge distillation made the student network optimized with fewer detours than the baseline network.
The metric $\rho$ measuring the stability of optimization directions was used to verify this hypothesis.


For image classification, natural language processing, and 3D point cloud classification,
Tables show that the student network usually had a larger $\rho$ value than the baseline network, which verified Hypothesis 3.
However, there was few failure cases.
When measuring $\rho$ by AlexNet and VGG-11, shallow architectures of these two networks lead to failure cases (please see discussions in Section~\ref{Verification of Hypothesis 2}).
There was also another failure case when we used the PointNet++ model to measure $\rho$, because this model was discriminative enough.
In this way, this PointNet++ model could make inferences based on a few knowledge points.




\subsection{Analysis of fine-tuning process}
We further checked whether knowledge points could be used to analyze other classic transfer-learning methods.
Here, we focused on fine-tuning a well-trained DNN on a new dataset.
Specifically, we conducted experiments to explore how the fine-tuning process guided the DNN to encode new knowledge points, where we fine-tuned a pre-trained VGG-16 network  on the Tiny ImageNet dataset.
Besides, we also trained another VGG-16 network from scratch on the same dataset  for comparison.
Figure shows that the fine-tuning process made the DNN learn new knowledge points in the foreground more quickly and be optimized with fewer detours than learning from scratch,~\textit{i.e.,} the fine-tuned DNN discarded fewer temporarily learned knowledge points.






\section{Conclusion and discussions}
This paper provides a new perspective to explain knowledge distillation from intermediate-layer features,
\textit{i.e.} quantifying knowledge points encoded in the intermediate layer of a DNN.
We propose three hypotheses on the mechanism of knowledge distillation, and design three types of metrics to verify these hypotheses in the scenario of different classification tasks.
Compared to learning from scratch, knowledge distillation ensures the DNN to encode more knowledge points, learn different knowledge points simultaneously, and optimize with fewer detours.
Note that the learning procedure of DNNs cannot be precisely divided into the learning phase and the discarding phase. In each epoch, the DNN may simultaneously learn new knowledge points and discard old knowledge points irrelevant to the task. Thus, the target epoch $\hat{m}$ in Figure is just a rough estimation of the division of two learning phases.



==> distill_check.tex <==



\section{abstract}
Compared to traditional learning from scratch, knowledge distillation sometimes makes the DNN achieve superior performance.
This paper provides a new perspective to explain the success of knowledge distillation, \textit{i.e.} quantifying knowledge points encoded in intermediate layers of a DNN for classification, based on the information theory.
To this end, we consider the signal processing in a DNN as the layer-wise information discarding.
A knowledge point is referred to as an input unit, whose information is much less discarded than other input units.
Thus, we propose three hypotheses for knowledge distillation based on the quantification of knowledge points.
\textbf{1.} The DNN learning from knowledge distillation encodes more knowledge points than the DNN learning from scratch. 
\textbf{2.} Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. In comparison, the DNN learning from scratch tends to encode various knowledge points sequentially.
\textbf{3.} The DNN learning from knowledge distillation is often optimized more stably than the DNN learning from scratch.
In order to verify the above hypotheses, we design three types of metrics with annotations of foreground objects to analyze feature representations of the DNN, \textit{i.e.} the quantity and the quality of knowledge points, the learning speed of different knowledge points, and the stability of optimization directions. 
In experiments, we diagnosed various DNNs for different classification tasks, \textit{i.e.} image classification, 3D point cloud classification, binary sentiment classification, and question answering, which verified above hypotheses.





\section{Introduction}
Knowledge distillation has achieved great success in various applications.
Knowledge distillation is referred to as the process of transferring the knowledge from one or more well-trained deep neural networks (DNNs), namely the teacher networks,
to a compact-yet-efficient DNN, namely the student network.
However, there have been very few studies to explain how and why knowledge distillation outperforms traditional learning from scratch.

Hinton owed the superior performance of knowledge distillation to the use of ``soft targets''.
Furlanello conjectured the effect of knowledge distillation on re-weighting training examples.
Lopez-Paz interpreted knowledge distillation as a form of learning with privileged information. 
Besides, from the perspective of network training, knowledge distillation was regarded as a label smoothing regularization method, and could enable faster convergence. 
These explanations for knowledge distillation were mainly based on qualitative statements or focused on the optimization and regularization effects.

Beyond the above perspectives for explanations, this paper provides a new perspective to analyze the success of knowledge distillation, \textit{i.e.} quantifying knowledge points encoded in the intermediate layer of a DNN. 
In other words, the quantity of knowledge points and the quality of knowledge points enable us to explain the representation power of the DNN, which is trained for classification.
For a better understanding, let us take the image classification as an example.
If a DNN learns lots of visual concepts for classification, then these concepts can be regarded as knowledge points, such as the bird head concept for the bird classification.
If these knowledge points are discriminative enough, then this DNN probably obtains good performance.


(a) Visualization of the information discarding through different layers of VGG-16 on the CUB200-2011 dataset. Input units with darker colors have less information discarding. 
 (b) Comparison of the coherency of different explanation methods. Our method coherently measures how input information is gradually discarded through layers, and enables fair comparisons of knowledge representations between different layers. In comparison, CAM and gradient explanations cannot generate coherent magnitudes of importance values through different layers for fair comparisons. More analysis is presented in Section.
  

The positive correlation between the ratio of foreground knowledge points $\lambda$ and the classification accuracy of DNNs on the CUB200-2011 dataset.}
   

In order to measure the quantity and the quality of knowledge points encoded in the DNN, we consider the signal processing in the forward propagation of a DNN as the process of layer-wise information discarding.
As Figure (a) shows, the DNN gradually discards the information of each input unit in the forward propagation. 
Here, an input unit is referred to as a variable (or a set of variables) in the input sample.
For example, the embedding of each word in the input sentence can be regarded as an input unit for natural language processing.
In the scenario of Figure (a), an input unit is referred to as a pixel (or pixels within a small local region) the input image.
Then, the information of some units (\textit{e.g.} information of pixels in the background) is discarded significantly.
In comparison, information of other input units (\textit{e.g.} information of pixels in the foreground) is less discarded.


In this way, we consider input units without significant information discarding as knowledge points, such as input units of the bird in Figure (a). 
These knowledge points usually encode discriminative information for inference, \textit{e.g.} wings of birds in Figure (a) are discriminative for the fine-grained bird classification.
In comparison, input units with significant information discarding usually do not contain discriminative information for prediction.
Thus, measuring the information discarding of input units enable us to quantify knowledge points.



Besides the quantity of knowledge points, we also measure the quality of knowledge points with the help of annotations of foreground objects.
To this end, we classify all knowledge points into two types, \textit{i.e.} knowledge points related to the task and knowledge points unrelated to the task.
In this way, we can compute the ratio of knowledge points encoded in a DNN that are relevant to the task, as a metric to evaluate the quality of knowledge points. 
A high ratio of relevant knowledge points indicates the feature representation of the DNN is reliable.
Figure shows that DNNs encoding a larger ratio of task-related knowledge points usually achieve better performance
(please see Section for more analysis).


Based on the quantification of knowledge points, we propose the following three hypotheses on reasons why knowledge distillation outperforms traditional learning from scratch. 
Furthermore, we design three types of metrics to verify these hypotheses.



\textbf{Hypothesis 1: Knowledge distillation makes the DNN learn more knowledge points than the DNN learning from scratch.} 
The information-bottleneck theory claimed that a DNN tended to preserve features relevant to the task and neglected those features irrelevant to the task for inference.
We assumed that a teacher network is supposed to achieve superior classification performance, because the teacher network usually has a complex network architecture or is often learned using more training data.
In this scenario, the teacher network is considered to encode more knowledge points related to the task and fewer knowledge points unrelated to the task than the student network.
In this way, knowledge distillation forces the student network to mimic the logic of the teacher network, which ensures the student network models more knowledge points relevant to the task and fewer knowledge points irrelevant to the task than the DNN learning from scratch.


\textbf{Hypothesis 2: Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. In comparison, the DNN learning from scratch tends to encode various knowledge points sequentially through different epochs.} 
It is because knowledge distillation forces the student network to mimic all knowledge points of the teacher network simultaneously.
In comparison, the DNN learning from scratch tends to focus on different knowledge points in different epochs sequentially.


\textbf{Hypothesis 3: Knowledge distillation usually yields more stable optimization directions than learning from scratch.}
The DNN learning from scratch usually keeps trying different knowledge points in early epochs and then discarding unreliable ones in late epochs, rather than model target knowledge points directly.
Thus, the optimization directions of the DNN learning from scratch is inconsistent. 
For convenience, in this paper, the phenomenon of inconsistent optimization directions through different epochs is termed as~\textbf{\textit{``detours''}}\footnote[1]{``Detours'' refer to the phenomenon that a DNN tends to encode various knowledge points in early epochs and discard non-discriminative ones later.}. 


Unlike learning from scratch, knowledge distillation usually forces the student network to mimic the teacher network directly.
The student network straightforwardly encodes target knowledge points without temporarily modeling and discarding other knowledge points.
Thus, the student network is optimized without significant detours.
For a better understanding of Hypothesis 3, let us take the fine-grained bird classification as an example. With the guidance of the teacher network, the student network directly learns discriminative features from heads or tails of birds without significant detours. In comparison, the DNN learning from scratch usually extracts features from the head, belly, tail, and tree-branch in early epochs, and later neglects features from the tree branch. In this case, the optimization direction of the DNN learning from scratch is more unstable.



Note that previous studies of explaining the optimization stability and the generalization power of the DNN were mainly from the perspective of the parameter space.
[1] demonstrated that the flatness of minima of the loss function resulted in good generalization. 
[2] illustrated that the generalization behavior of the network depended on the norm of the weights.
In contrast, this paper explains the efficiency of optimization from the perspective of knowledge representations, \textit{i.e.} analyzing whether or not the DNN encodes different knowledge points simultaneously and without significant detours.



\textbf{Connection to the information-bottleneck theory.}
We roughly consider that the information-bottleneck theory can also be used to explain the change of knowledge points in a DNN. It showed that a DNN usually extracted a few discriminative features for inference, and neglected massive features irrelevant to the inference during the training process.
The information-bottleneck theory measures the entire discrimination power of each sample.
In comparison, our method quantifies the discrimination power of each input unit in a more detailed manner, and measures pixel-wise information discarding through forward propagation.


\textbf{Methods.} 
In order to verify above hypotheses, we design three types of metrics to quantify knowledge points encoded in intermediate layers of a DNN, and analyze how different knowledge points are modeled during the training procedure. 


$\bullet\quad$The first type of metrics measures the quantity and quality of knowledge points.
We consider that a well-trained DNN with superior classification performance is supposed to encode
massive knowledge points, where most knowledge points are discriminative for the classification of target categories.

$\bullet\quad$The second type of metrics measures whether a DNN encodes various knowledge points simultaneously or sequentially, \textit{i.e.} examining whether different knowledge points are learned at similar speeds.

$\bullet\quad$The third metric evaluates whether a DNN is optimized with or without significant detours.
In other words, this metric measures whether or not the DNN directly learns target knowledge points without temporarily modeling and discarding other knowledge points.
To this end, this metric is designed as the overlap between knowledge points encoded by the DNN in early epochs and final knowledge points of the DNN.
If this overlap is large, then we consider this DNN is optimized without significant detours; otherwise, with detours.
It is because a small overlap indicates that 
the DNN first encodes a large number of knowledge points in early epochs, but many of these knowledge points are discarded in later epochs.

In summary, we use these metrics to compare knowledge distillation and learning from scratch, in order to verify Hypotheses 1-3. 

\textbf{Using the annotated knowledge points or not.}
In particular, we should define and quantify knowledge points without any human annotations.
It is because we do not want the analysis of the DNN to be influenced by manual annotations with significant subjective bias, which hurts the trustworthiness of this research.
Besides, the cost of annotating all knowledge points is also unaffordable.
However, previous studies often define visual concepts (knowledge points) by human annotations, and these concepts usually have specific semantic meanings.
For example, Bau manually annotated six types of semantic visual concepts (objects, parts, textures, scenes, materials, and colors) to explain feature representations of DNNs.
In this way, these methods cannot fairly quantify the actual amount of knowledge encoded by a DNN, because most visual concepts are not countable and cannot be defined with human annotations.

In contrast, this paper uses the information discarding of each input unit to define and quantify knowledge points without human annotations.
Such knowledge points are usually referred to as \textit{\textbf{``Dark Matters'' }}.
Compared to traditionally labeled visual concepts, we consider these dark-matter knowledge points can provide a more general and trustworthy way to explain feature representations of DNNs.


\textbf{Scope of explanation.}
A trustworthy explanation of knowledge distillation usually has two requirements.
First, the teacher network is supposed to be well optimized as the student network.
Otherwise, if the teacher network does not converge or is optimized for other tasks, then the teacher network is not qualified for distillation.
Second, knowledge distillation often has two fully different utilities. 
(1) Distilling from high-dimensional features usually forces the student network to mimic all sophisticated feature representations in the teacher network.
(2) Distilling from the low-dimensional network output mainly selectively uses confident training samples for learning, 
with very little information on how the teacher encodes detailed features. 
In this case, the distillation selectively emphasizes the training of simple samples and ignores the training of hard samples\footnote[2]{Confident (simple) samples usually generate salient output signals for knowledge distillation than unconfident (hard) samples.}.
Therefore, in this paper, we mainly explain the first utility of knowledge distillation, 
\textit{i.e.,} forcing the student network to mimic the knowledge of the teacher network.
Such a utility is  mainly exhibited by distilling from high-dimensional intermediate-layer features.


Contributions of this paper are summarized as follows.

1. The quantification of knowledge points encoded in intermediate layers of DNNs can be used as a new perspective to analyze DNNs.

2.  Based on the quantification of knowledge points, we design three types of metrics to explain the mechanism of knowledge distillation.

3. Three hypotheses about knowledge distillation are proposed and verified in different classification applications, including image classification, 3D point cloud classification, binary sentiment classification, and question answering,
which shed new light on the interpretation of knowledge distillation.

A preliminary version of this paper appeared in [1].




\section{Related work}
Although DNNs have shown promises in various applications, they are still regarded as black boxes. Previous studies of interpreting DNNs are roughly summarized as semantic explanations and mathematical analysis of the representation capacity.

$\bullet\quad$\textbf{Semantic explanations for DNNs.} 
An intuitive way to explain DNNs is to visualize the appearance encoded in intermediate layers of DNNs, which may significantly activate a specific neuron of a certain layer. Gradient-based methods measured the importance of intermediate-layer activation units or input units by using gradients of outputs \textit{w.r.t.} inputs. Inversion-based methods  inverted feature maps of convolutional  layers into images. 
Moreover, some studies estimated the pixel-wise or regional attribution/importance/saliency of an input to the network output.

The semantic dissection is also a classical direction of interpreting DNNs. 
Bau manually annotated six types of visual concepts (\textit{objects, parts, scenes, textures, materials} and \textit{colors}), and associated units of DNN feature maps with these concepts. 
Furthermore, the first two concepts could be summarized as shapes, and the last four concepts could be summarized as textures. 
Fong and Vedaldi used a set of filters to represent a single semantic concept, and built up many-to-many projections between concepts and filters. 
TCAV measured the importance of user-defined concepts to classification results.

Learning a DNN with interpretable feature representations in an unsupervised or weakly-supervised manner is another direction of explainable AI. 
InfoGAN and $\beta$-VAE learned interpretable latent representations for generative networks. 
In the capsule network, each capsule encoded different meaningful features. 
Interpretable CNNs were used to make each filter in a high convolutional layer represent a specific object part.  
The BagNet was proposed to classify images based on the occurrences of local image features. 
The ProtoPNet  was introduced to learn prototypical parts.
Shen proposed a method to modify a traditional CNN into an
interpretable compositional CNN.

In summary, previous studies are mainly based on heuristic assumptions to calculate importance/saliency/attention or use massive human-annotated concepts to interpret network features. 
Whereas, in this paper, we explain feature representations from the perspective of knowledge points.


$\bullet\quad$\textbf{Mathematical explanations for the representation capacity of DNNs.} 
Formulating and evaluating the representation capacity of DNNs is an emerging direction of explainable AI. 
The information-bottleneck theory provided a generic metric to quantify the information encoded in DNNs, which can be extended to evaluate the representation capacity of DNNs. 
Zhang discussed the relationship between the parameter number and the generalization capacity of DNNs. 
Weng proposed to use the CLEVER score to measure the robustness of neural networks. 
Fort used the stiffness to diagnose the generalization of a DNN.
The module criticality was proposed to explain the superior generalization performance of some network architectures.

Unlike previous studies, this paper aims to bridge the gap between mathematical explanations and semantic explanations. In other words, we use the information discarding of the input to quantify knowledge points and to explain the discrimination power of the DNN. More specifically, we analyze the quantity and the quality of knowledge points in a DNN, measure whether a DNN encodes various knowledge points sequentially or simultaneously, and evaluate the stability of optimization direction.


$\bullet\quad$\textbf{Knowledge distillation.} 
Knowledge distillation is a popular technique in knowledge transferring, which can be applied to different domains such as adversarial defense, object detection, semantic segmentation, model compression, and improving generalization. 

Although knowledge distillation has achieved success in various applications, there have been very few attempts on explaining how and why it helps the training of the DNN. Hinton demonstrated that learning from ``soft targets'' was easier than learning from ``hard targets".
Furlanello explained the efficiency of knowledge distillation as re-weighting training examples.
From a theoretical perspective, Lopez-Paz related knowledge distillation to learning from privileged information under a noise-free setting.  
Phuong and Lampert explained the success of knowledge distillation from the view of data distribution, optimization bias, and the size of the training set. 
Yuan interpreted knowledge distillation in terms of Label Smoothing Regularization. 
Menon considered that a good teacher modeling the Bayes class-probabilities resulted in the success of knowledge distillation.

However, previous explanations for knowledge distillation were mainly based on 
qualitative statements or theoretically relied on strong assumptions, such as linear models.
In contrast, we interpret knowledge distillation from the perspective of knowledge representations, \textit{i.e.} quantifying, analyzing, and comparing knowledge points encoded in distilled DNNs and knowledge points encoded in DNNs learning from scratch.
Hence, knowledge points provide new insight into the success of knowledge distillation.




\section{Algorithm}
In this paper, we explain the success of knowledge distillation from a new perspective, \textit{i.e.} quantifying knowledge points encoded in the intermediate layers of a DNN for classification.
Unlike previous explanations for knowledge distillation, our method enables people to explain the representation power of a DNN using the quantity and the quality of knowledge points encoded in a DNN, which reflects a more direct and stronger connection between the knowledge and the performance.
To this end, we measure the information discarding of each input unit to define knowledge points in a DNN, based on the information theory.
We propose three hypotheses on the mechanism of knowledge distillation to explain its success.
In order to verify these hypotheses, we further design three types of metrics based on the quantification of knowledge points, which evaluate the representation quality of the DNN.
Note that theoretically, knowledge distillation usually has two fully different utilities.
Distillation from high-dimensional intermediate-layer features usually exhibits the first type of utilities,~\textit{i.e.,} forcing the student network to mimic knowledge points of the teacher network.
Whereas, distilling from relatively low-dimensional network output often exhibits the second type of utilities,~\textit{i.e.,} selecting confident samples for learning and ignoring  unconfident samples.
In this paper, we mainly explain the first utility of knowledge distillation, which is mainly exhibited by distilling from high-dimensional intermediate-layer features.


\subsection{Quantifying Information Discarding}
Before defining and quantifying knowledge points encoded in DNNs, we first introduce how to measure the pixel-wise information discarding of the input sample in this section.

According to information-bottleneck theory, we consider the signal processing of a forward propagation as the layer-wise discarding of input information.
In low layers, most input information is used to compute features.
Whereas, in high layers, information in input units unrelated to the inference is gradually discarded, and only related pixel-wise information is maintained in the computation of network features.
In this way, we consider features of the highest layer mainly encode the information, which is highly relevant to the inference.

Thus, we propose methods to quantify the input information encoded in a specific intermediate layer of a DNN, \textit{i.e.} measuring how much input information is discarded when the DNN extracts the feature of this layer.
 To this end, the information discarding of each input unit is formulated as the entropy, given a feature of a certain network layer.
 
Specifically, given a trained DNN for classification and an object instance $x\in{R^{n}}$ with $n$ input units, let $f^{*}=f(x)$ denote the feature of a network intermediate layer, 
and let $y^{*}$ denote the network prediction~\textit{w.r.t.} $x$.
The input unit is referred to as a variable (or a set of variabels) in the input sample.
For example, each pixel (or pixels within a small local region) of an input image can be taken as an input unit, 
and the embedding of each word in an input sentence also can be regarded as an input unit.


In our previous works, 
we consider that the DNN satisfies the Lipschitz constraint
$\parallel{y'-y^{*}}\parallel \le \kappa \parallel{f(x')-f^{*}}\parallel^{2}$, where $\kappa$ is the Lipschitz constant, and $y'$ corresponds to the network prediction of the sample $x'$.
The  Lipschitz constant $\kappa$ can be computed as the maximum norm of the gradient within a small range of features,~\textit{i.e.,}
{\small$\kappa = \max_x \parallel{\nabla f(x)}\parallel$}.
In fact, for any continuous function without a singular point, there often exists a Lipschitz constant for this function.
Besides, many previous studies assumed that a DNN has such a specific Lipschitz constant.
This indicates that 
If we add a small perturbation to the intermediate-layer feature, then the change of the DNN's output is also limited,~\textit{i.e.,} $\parallel{y'-y^{*}}\parallel \le \delta f$.
In other words,
the DNN usually represents a specific object instance using a very limited range of features $\small{ \parallel{f(x')-f^{*}}\parallel ^{2}\le \tau}$, where $\tau$ is a  positive scalar and $f(x')$ denotes the feature in the limited range.
In other words, all features in $\small{\{f(x')\big{|} \parallel{f(x')-f^{*}}\parallel ^{2}\le \tau\}}$ represent the same object instance, 
\textit{i.e.}, $\small{\parallel{y'-y^{*}}\parallel \le \kappa \cdot \tau}$.


However, it is very difficult to determine the explicit low-dimensional manifold of features \textit{w.r.t.} the input $x$.
As an expediency, we add perturbations $\Delta x$ to the input sample $x$ to approximate the manifold of the feature, \textit{i.e.} generating samples 
$x'= x+\Delta x$, subject to
$\small{ \parallel{f(x')-f^{*}}\parallel ^{2}\le \tau}$.
In this way, the entropy $H(X')$ measures the uncertainty of the input when the feature represents the same object instance, 
$\small{\parallel{y'-y^{*}}\parallel \le \kappa \cdot \tau}$, as mentioned above.
In other words, $H(X')$ quantifies how much input information can be discarded without affecting the inference of the object.
$X'$ denotes a set of inputs corresponding to the concept of a specific object instance. 
It is assumed that $\Delta x$ is an \textit{i.i.d.} Gaussian noise, thereby $x'= x+\Delta x \sim \mathcal{N}(x,\Sigma(\boldsymbol\sigma) = diag(\sigma_{1}^{2},\dots, \sigma_{n}^{2}))$.
Here, $\sigma_{i}$ indicates the variance of the perturbation \textit{w.r.t.} the $i$-th input unit.
The assumption of the Gaussian distribution ensures that the entropy $H(X') $ of the input can be decomposed into pixel-level entropies $\{H_{i}\}$.
\begin{equation}\label{2}
\small{H(X') = \sum_{i=1}^{n} H_{i},}
\end{equation}
where $H_{i} = \log\sigma_{i} +  \frac{1}{2} \log(2\pi{e})$ measures the pixel-wise information discarding. 
A large value of $H_{i}$ usually indicates that the information of the $i$-th unit is significantly discarded during the forward propagation.
For example, as Figure~\ref{fig:layer}(a) shows, information encoded in background pixels is significantly discarded for the fine-grained bird classification.



Thus, we learn the optimal $\Sigma(\boldsymbol\sigma) = diag(\sigma_{1}^{2},\dots, \sigma_{n}^{2})$ via the maximum-entropy principle to compute the pixel-wise information discarding $H_{i}= \log\sigma_{i} +  \frac{1}{2} \log(2\pi{e})$.
The objective function is formulated in Equation, which maximizes $H(X')$ subject to constraining features within the scope of a specific object instance $\small{\parallel{f(x')-f^{*}}\parallel ^{2}\le \tau}$.
\textit{I.e.,} we enumerate all perturbation directions in the input sample $x$ within a small variance of the feature $f^{*}$, in order to approximate the low-dimensional manifold of $f(x')$. 
We use the Lagrange multiplier to approximate Equation as the following loss.
Considering Equation is intractable, we use $x'=x+{\boldsymbol\sigma}\circ{\boldsymbol\delta}, \delta\sim\mathcal{N}(0,I)$ to simplify the computation of $\text{Loss}({\boldsymbol\sigma})$, where {\small$\circ$} denotes the element-wise multiplication.
{\small${\boldsymbol\sigma}=[\sigma_1,\ldots,\sigma_{n}]^{\top}$} represents the range that the input sample can change.
In this way, $\text{Loss}({\boldsymbol\sigma})$ in Equation is tractable, and we can learn $\boldsymbol\sigma$ via gradient descent.
{\small $\delta_f^2 = \lim_{\tau\rightarrow0^{+}}\mathbb{E}_{x'\sim\mathcal{N}(x,\tau{^2} I )}\left[\Vert f(x')-f^{*}\Vert^2\right]$} denotes the inherent variance of intermediate-layer features subject to small input noises with a fixed magnitude $\tau$. $\delta_f^2$ is used for normalization, and a positive scalar $\alpha$ is used to balance the two loss term.




\subsection{Quantification of knowledge points}
\textbf{Hypothesis 1}: Knowledge distillation makes the DNN encode more knowledge points than learning from scratch.




The basic idea is to measure the quantity and quality of knowledge points encoded in intermediate layers of a DNN.



Visualization of knowledge points. The dark color indicates the low entropy value ${H_{i}}$. Image regions with low pixel-wise entropies ${\{H_{i}\}}$ are considered as knowledge points. In real implementation, to improve the stability and efficiency of the computation, we divide the image into $16\times16$ grids, and each grid is taken as a ``pixel" to compute the entropy $H_{i}$.





$\bullet\quad$\textbf{The quantity of knowledge points.}
In this paper, we use the pixel-wise information discarding of each input unit to define and quantify knowledge points.
Given a trained DNN and an input sample $x \in X$, let us focus on the pixel-wise information discarding ${H_{i}}$ \textit{w.r.t.} the feature of a certain network layer $f^{*}=f(x)$.
$X$ represents a set of input samples.

According to Equation~\eqref{2}, a low pixel-wise entropy $H_{i}$ represents the information of this input unit is less discarded.
In other words, the DNN tends to use these input units with low entropies to compute the feature $f^{*}$ and make the inference.
Thus, a knowledge point is defined as an input unit with a low pixel-wise entropy $H_{i}$, which encodes discriminative information for prediction.
For example, bird heads in Figure~\ref{fig1} are referred to as knowledge points, which are useful for the fine-grained bird classification.

To this end, we use the average entropy $\overline{H}$ of all background units $\Lambda_{\textrm{bg}}$ as a baseline to determine knowledge points, \textit{i.e.} $\overline{H}=\mathbb{E}_{i \in \Lambda_{\textrm{bg}}}[H_{i}]$.
It is because information encoded in background units is usually supposed to be significantly discarded and irrelevant to the inference.
If the entropy of a unit is significantly lower than the baseline entropy $\overline{H} - H_{i} > b$, then this input unit can be considered as a valid knowledge point.
Here, $b$ is a threshold to determine the knowledge points, which is introduced in Section~\ref{Implementation Details}.
In this way, we can quantify the number of knowledge points in the DNN.

$\bullet\quad$\textbf{The quality of knowledge points.}
Besides the quantity of knowledge points, we also consider the quality of knowledge points.
Generally speaking, information encoded in foreground units is usually supposed to be crucial to the inference.
In comparison, information encoded in background units is often supposed to have negligible effects on the prediction.
Therefore, we design a metric $\lambda$ to evaluate the quality of knowledge points by examining whether or not most knowledge points are localized in the foreground.
$N_{\textrm{point}}^{\textrm{bg}}(x)$ and $N_{\textrm{point}}^{\textrm{fg}}(x)$ denote the number of knowledge points encoded in the background and the foreground, respectively.
$\Lambda_{\textrm{bg}}$ and $\Lambda_{\textrm{fg}}$ are sets of input units in the background and the foreground \textit{w.r.t.} the input sample $x$, respectively.
$\mathbbm{1}(\cdot)$ refers to the indicator function. If the condition inside is valid, then $\mathbbm{1}(\cdot)$ returns $1$; otherwise, returns $0$.
A large value $\lambda$ represents the feature representation of the DNN is reliable; otherwise, unreliable.

Thus, knowledge points provide a new way to explain the mechanism of knowledge distillation, \textit{i.e.} checking whether or not knowledge distillation makes the DNN encode massive knowledge points, and whether or not most knowledge points are precisely localized in the foreground.




Comparisons of different explanation methods in terms of the coherency. The coherency of the entropy-based method enables fair layer-wise comparisons within a network, and fair comparisons between different networks.




\textbf{Coherency and generality}.
As discussed in [1], a trustworthy explanation method to evaluate feature representations of the DNN should satisfy criteria of the coherency and generality.
From this perspective, we analyze the trustworthiness of knowledge points.

The \textbf{coherency} indicates the explanation method should reflect the essence of the encoded knowledge representations in DNNs, which are invariant to network settings.
In this paper, we use pixel-wise information discarding to define knowledge points without strong assumptions of feature representations, or network architectures.
In this way, knowledge points yield a coherent evaluation of feature representations.
However, most existing explanation methods in Table usually fail to meet this criterion due to their biased assumptions. 
For example, the CAM and gradient explanations do not generate coherent explanations, because the gradient map $\frac{\partial Loss}{\partial f}$ is usually not coherent through different layers.

To this end, we compare our method with  the CAM and the gradient explanations.
Theoretically, we can easily construct two DNNs representing exactly the same knowledge but with different magnitudes of gradients, as follows.
A VGG-16 model was learned using the CUB200-2011 dataset for fine-grained bird classification.
Given this pre-trained DNN, we slightly revised the magnitude of parameters in every pair of neighboring convolutional layers {\small$y=x\otimes w+b$} to examine the coherency.
For the {\small$L$}-th and {\small$(L+1)$}-th layers, parameters were revised as {\small$w^{(L)}\leftarrow 4w^{(L)}$}, {\small$w^{(L+1)}\leftarrow w^{(L+1)}/4$}, {\small$b^{(L)}\leftarrow 4b^{(L)}$}, {\small$b^{(L+1)}\leftarrow b^{(L+1)}/4$}.
Such revisions did not change knowledge representations or the network output, but changed the gradient magnitude.

As Figure (b) shows, magnitudes of the CAM and the gradient explanation methods are sensitive to the magnitude of parameters. In comparison, our method is not affected by the magnitude of parameters, which demonstrates the coherency. Thus, the coherency of our method enables fair layer-wise comparisons within a DNN, and fair comparisons between different DNNs.

The \textbf{generality} means that the explanation method should have strong connections to existing mathematical theories.
To this end, we quantify knowledge points using the entropy of the input sample.
The entropy is a generic tool with strong connections to various theories, \textit{e.g.} the information-bottleneck theory.
As a result, the generality of knowledge points enables us to fairly compare feature representations between different DNNs.
Note that calculating knowledge points requires the annotation of the foreground, but this requirement does not hurt the coherency and the generality of knowledge points.




\subsection{Learning simultaneously or sequentially}
\textbf{Hypothesis 2}: Knowledge distillation makes the DNN more likely to learn different knowledge points simultaneously. Whereas, the DNN learning from scratch tends to encode various knowledge points sequentially in different epochs.



Procedure of learning foreground knowledge points \textit{w.r.t.} weight distances. According to information-bottleneck theory, a DNN tends to learn various knowledge points in early epochs and then discard knowledge points irrelevant to the task later. Strictly speaking, a DNN learns new knowledge points and discards old ones during entire the learning process. The epoch $\hat{m}_{x}$ encodes the richest foreground knowledge points.}





This hypothesis can be understood as follows.
Knowledge distillation forces the student network to mimic all knowledge points of the teacher network simultaneously.
In comparison, the DNN learning from scratch is more likely to learn different knowledge points in different epochs.
A DNN learning from scratch may encode knowledge points of common, simple, and elementary features in early epochs.
For example, in the scenario of fine-grained bird classification, the sky is a typical and simple feature to learn.
Whereas, knowledge points representing complex features may be encoded in later epochs by the DNN learning from scratch.
For example, in the scenario of fine-grained bird classification, the subtle difference between two similar bird species is difficult to learn.
In this way, the DNN learning from scratch tends to encode different knowledge points in a sequential manner, rather than simultaneously.

\textbf{Metrics.}
In order to verify Hypothesis 2, we design two metrics, which examines whether or not 
different knowledge points are learned within similar epochs, \textit{i.e.} whether or not learning different knowledge points simultaneously.

Specifically, given a set of training samples $X$, let $M$ denote the total epochs to train a DNN.
For each specific sample $x\in X$, foreground knowledge points learned by DNNs after $j$ epochs are represented as 
$N_{j}^{\textrm{fg}}(x)$, where $j \in \{1,2,\cdots,M\}$.

In this way, whether or not a DNN learns different knowledge points simultaneously can be measured from the following two aspects.
(1) Whether or not the number of foreground knowledge points $N_{j}^{\textrm{fg}}(x)$ increases fast along with the epoch number.
(2) Whether or not $N_{j}^{\textrm{fg}}(x)$~\textit{w.r.t.} different samples increase simultaneously.
In other words, the first aspect measures whether or not the DNN learns various knowledge points of a specific input sample quickly, and the second aspect evaluates whether a DNN learns knowledge points of different samples at similar speeds.

To this end, as Figure shows, we consider the epoch $\hat{m}$ that a DNN obtains richest foreground knowledge points to measure the learning speeds, 
\textit{i.e.} $\hat{m}_{x} = \arg\max_{k} N_{k}^{\textrm{fg}}(x)$.
We use metrics $D_{\textrm{mean}}$ and $D_{\textrm{var}}$ based on the \textit{``weight distance'' } $\sum_{k=1}^{{m}} \frac{\|{w_{k}-w_{k-1}}\|}{\|{w_{0}}\|}$ to check whether a DNN learns knowledge points simultaneously or not.
$w_{0}$ and $w_{k}$ denote initial parameters and parameters learned after the $k$-th epoch, respectively.
The metric $D_{\textrm{mean}}$ represents the average weight distance that the DNN obtains the richest foreground knowledge points, and
the metric $D_{\textrm{var}}$ describes the variation of the weight distance \textit{w.r.t.} different input samples.
These two metrics are defined as follows.
Here, we use the weight distance  to evaluate the learning effect at each epoch, rather than use the epoch number.
It is because the weight distance better quantifies the total path of updating the parameter $w_{k}$ at each epoch $k$ than the epoch number.
In other words, the weight distance can better measure the dynamic learning process of the DNN.
In this way, $D_{\textrm{mean}}$ measures whether a DNN learns knowledge points quickly, and $D_{\textrm{var}}$ evaluates whether a DNN learns knowledge points of different input samples at similar speeds.
Thus, small values of $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ reflect that the DNN learns various knowledge points quickly and simultaneously.







\subsection {Learning with Less Detours}
\textbf{Hypothesis 3}: Knowledge distillation usually yields more stable optimization directions than learning from scratch.



Detours of learning knowledge points. We visualize sets of foreground knowledge points learned after different epochs. The green box indicates the union of knowledge points learned during all epochs. The $(1-\rho)$ value denotes the ratio of knowledge points that are discarded during the learning process to the union set of all learned knowledge points. A larger $\rho$ value indicates DNN is optimized with fewer detours.
    


This hypothesis can be understood as follows.
According to the information-bottleneck theory, the DNN learning from scratch usually tries to model various knowledge points in early epochs and then discards those unrelated to the inference in late epochs.
It means that the DNN learning from scratch cannot directly encode target knowledge points for inference.
Thus, the optimization direction of this DNN is inconsistent and unstable in early and late epochs, \textit{i.e.} with significant detours.
Unlike learning from scratch, knowledge distillation forces the student network to directly mimic the well-trained teacher network.
With the guidance of the teacher network, knowledge distillation makes the student network straightforwardly model target knowledge points without temporarily modeling and discarding other knowledge points.
Thus, the DNN learning via knowledge distillation tends to be optimized in a stable direction, \textit{i.e.} without significant detours.


\textbf{Metric.}
In order to verify Hypothesis 3, we design a metric to evaluate whether a DNN is optimized in a stable and consistent direction or not.
Let $S_{j}(x)=\{i\in x|\overline{H} - H_{i} > b\}$ denote the set of foreground knowledge points in the input sample $I$ encoded by the DNN learned after the $j$-th epoch, where $j\in\{1,2,\cdots,M\}$.
Each knowledge point $a \in{S_{j}(x)}$ is referred to as a specific unit $i$ on the foreground of the input sample $I$, which satisfies $\overline{H} - H_{i} > b$. 
Then, we use the metric $\rho$ to measure the stability of optimization directions.
$\rho$ represents the ratio of finally encoded knowledge points to all temporarily tried knowledge points in intermediate epochs, where $|\cdot|$ denotes the cardinality of the set.
More specifically, the numerator of Equation reflects the number of foreground knowledge points, which have been chosen ultimately for inference.
For example, knowledge points in the black box of Figure are encoded as final knowledge points for the fine-grained bird classification.
The denominator represents the number of all knowledge points temporarily learned during the entire training process, which is shown as the green box in Figure.
Moreover, $(\bigcup_{j=1}^{M} S_{j}(x)\setminus{S_{M}(x))}$ indicates a set of knowledge points, which have been tried, but finally are discarded by the DNN. 
The set of those discarded knowledge points is shown as the brown box in Figure.
Thus, a high value of $\rho$ indicates that the DNN is optimized without significant detours and more stably; otherwise, with significant detours.



\section{Experiment}
In this section, we conducted comparative experiments on image classification, 3D point cloud classification, and natural language processing (NLP) tasks. These experiments verified the proposed hypotheses.




\subsection{Implementation Details}
Given a teacher network, we distilled knowledge from the teacher network to the student network.
In order to remove the effects of network architectures, the student network had the same architecture as the teacher network.
Meanwhile, for fair comparisons, the DNN learning from scratch was also required to have the same architecture as the teacher network.
For convenience,  we named the DNN learning from scratch the \textbf{baseline network} in the following manuscript. 



Additionally, we conducted experiments to check whether the size of the teacher network hurt the verification of three hypotheses.
Tables show when the student network distilled from a larger teacher network, Hypotheses 1-3 were still verified.
This phenomenon indicates that the change of teacher network size did not hurt the verification of our conclusions.
To simplify the story, we set student networks to have the same architectures as teacher networks in the following experiments.



Comparisons between the student network and the baseline network (B) for the image classification on the CUB200-2011 dataset, where student network distilled from $\textrm{FC}_{1}$ layer of a larger teacher network.




Comparisons between the student network (S) and the baseline network (B) for image classification on the CUB200-2011 dataset, respectively. 
Metrics were evaluated at the $\textrm{FC}_{1}$ layer under different settings of the grid size and different settings of the threshold $b$. Experimental results verified Hypotheses 1-3.





\textbf{Datasets \& DNNs.} 
\textit{For the image classification task}, we conducted experiments based on AlexNet, VGG-11, VGG-16, VGG-19, ResNet-50, ResNet-101, and ResNet-152. 
We trained these DNNs based on the ILSVRC-2013 DET dataset, the CUB200-2011 dataset, and the Pascal VOC 2012 dataset for object classification, respectively. 
Considering the high computational burden of training on the entire ILSVRC-2013 DET dataset, we conducted the classification of terrestrial mammal categories for comparative experiments.
Note that all teacher networks were pre-trained on the ImageNet dataset, and then fine-tuned using the aforementioned dataset. 
In comparison, all baseline networks were learned from scratch. 
Moreover, data augmentation was applied to 
both the student network and the baseline network, when DNNs were learned using the ILSVRC-2013 DET dataset or the Pascal VOC 2012 dataset.


We used object images cropped by object bounding boxes to train the aforementioned DNNs on each above dataset, respectively.
In particular, to achieve stable results, images in the Pascal VOC 2012 dataset were cropped by using $1.2 \,{width} \times 1.2 \,{height}$ of the original object bounding box. 
For the ILSVRC-2013 DET dataset, we cropped each image by using $1.5 \,{width} \times 1.5 \,{height}$ of the original object bounding box. 
It is because there existed no ground-truth annotations of object segmentation for the ILSVRC-2013 DET dataset.
We used the object bounding box to separate foreground regions and background regions of images in the ILSVRC-2013 DET dataset.
In this way, pixels within the object bounding box were regarded as the foreground~$\Lambda_{\textrm{fg}}$, and pixels outside the object bounding box were referred to as the background~$\Lambda_{\textrm{bg}}$.

\textit{For natural language processing}, we fine-tuned a pre-trained BERT model using the SQuAD dataset as the teacher network towards question answering.
Besides, we also fine-tuned another pre-trained BERT model on the SST-2 dataset as the teacher network for binary sentiment classification.
Baseline networks and student networks were just trained using samples in the SST-2 dataset or the SQuAD dataset.
Moreover, for both the SQuAD dataset and the SST-2 dataset, we annotated input units irrelevant to the prediction as the background~$\Lambda_{\textrm{bg}}$, according to the human cognition.
We annotated units relevant to the inference as the foreground~$\Lambda_{\textrm{fg}}$.
For example, words related to answers were labeled as foregrounds in the SQuAD dataset. Words containing sentiments were annotated as foregrounds in the SST-2 dataset.

\textit{For 3D point cloud classification task}, we conducted comparative experiments on the PointNet, DGCNN, PointConv, and PointNet++ models.
Considering most widely used benchmark datasets for point cloud classification only contained foreground objects, we constructed a new dataset containing both foreground objects and background objects based on the ModelNet40 dataset, as follows.
For each sample (\textit{i.e.} the foreground object) in the ModelNet40 dataset, 
we first randomly sampled five point clouds, whose labels are different from the foreground object. 
Then, we randomly selected $500$ points from the sampled five point clouds, and attached these points to the foreground object as background points.
Moreover, the teacher network was trained using all training data in this generated dataset for classification.
In comparison, we only randomly sampled $10\%$ training data in this generated dataset to learn baseline networks and student networks, respectively.
Thus, the teacher network was ensured to encode better knowledge representations.



\textbf{Distillation.} 
Given a well-trained teacher network and an input sample $x$, we selected a convolutional layer or a fully-connected (FC) layer $l$ as the target layer to perform knowledge distillation.
We used the distillation loss $\|f_{T}(x)-f_{S}(x)\|^{2}$ to force the student network to mimic the feature of the teacher network.
Here, $f_{T}(x)$ denoted the feature of $l$-th layer in the teacher network, and $f_{S}(x)$ indicated the feature of $l$-th layer in its corresponding student network.


In order to simplify the story, we used the distillation loss to learn the student network, rather than the classification loss.
Given the distilled features, we further learned parameters above the target layer $l$ merely using the classification loss.
In this way, we could ensure that all knowledge points of student network were exclusively learned via distillation.
Otherwise, if we trained the student network using both the distillation loss and the classification loss, then it would be hard to distinguish whether the classification loss or the distillation loss was responsible for the learning of each knowledge point. 



Moreover, we employed two schemes of knowledge distillation in this paper,~\textit{i.e.} learning from intermediate-layer features and learning from network output.
Specifically, 
we distilled features in the top convolutional layer ($\textrm{Conv}$) or in each of three FC layers (namely $\textrm{FC}_{1}$, $\textrm{FC}_{2}$ and $\textrm{FC}_{3}$) of the teacher network to train the student network, respectively.
In this way, knowledge distillation from the $\textrm{FC}_{3}$ layer corresponded to the scheme of learning from output, and distillation from other layers corresponded to the scheme of learning from intermediate-layer features.
In spite of these two schemes, we mainly explained knowledge distillation from intermediate-layer features 
that forced the student network to mimic the knowledge of the teacher network as discussed before.



\textbf{The layer used to quantify knowledge points.} 
For each pair of the student network and the baseline network, we measured knowledge points on the top convolutional layer and all FC layers.

Particularly, for DNNs learned on the ILSVRC-2013 DET dataset and the Pascal VOC 2012 dataset, we quantified knowledge points only on $\textrm{FC}_{1}$ and $\textrm{FC}_{2}$ layers,
because the dimension of features in the output layer $\textrm{FC}_{3}$ was much fewer than that of intermediate-layer features in the $\textrm{FC}_{1}$ and $ \textrm{FC}_{2}$ layers.
Similarly, for DNNs trained on the ModelNet40 dataset, we also used the $\textrm{FC}_{1}$ and $ \textrm{FC}_{2}$ layers to quantify knowledge points.
For the BERT model, we measured knowledge points on its last hidden layer.
Considering ResNets usually only had one FC layer, to obtain rich knowledge representations, we added two $\textrm{Conv}$ layers and two FC layers before the last FC layer.
In this way, we quantified knowledge points on these three FC layers.




\textbf{Hyper-parameter settings.}
We used the SGD optimizer, and set the batch size as 64 to train DNNs. 
We set grid size to $16 \times 16$, and settings of the threshold $b$ was as follows.
For DNNs towards image classification, $b$ was set to $0.2$, except that we set $b$ to $0.25$ for AlexNet.
For BERT towards NLP tasks, $b$ was set to $0.2$.
For DNNs towards 3D point cloud classification,  $b$ was set to $0.25$, besides that $b$ was set to $0.5$ for PointNet.


Additionally, we also tested the influence of the grid size and the threshold $b$ on the verification of the three hypotheses.
To this end, we conducted experiments with different settings of the grid size and different settings of the threshold $b$.
Table~\ref{tab:grid_size_b} shows that Hypotheses 1-3 were still validated, when knowledge points were calculated under different different settings of the grid size and different settings of the threshold $b$.



Comparisons of knowledge points encoded in the teacher network (T), the student network (S) and the baseline network (B) for image classification. The teacher network encoded more foreground knowledge points $N_{\textrm{point}}^{\textrm{fg}}$ and obtained a larger ratio $\lambda$ than the student network. Meanwhile, the student network had larger values of $N_{\textrm{point}}^{\textrm{fg}}$ and $\lambda$ than  baseline network.


Visualization of knowledge points encoded in the $ \textrm{FC}_{1}$ layer of VGG-11. Generally, the student network  had a larger $N_{\textrm{point}}^{\textrm{fg}}$ value and a smaller $N_{\textrm{point}}^{\textrm{bg}}$ value than the baseline network.



Comparisons between the student network (S) and the baseline network (B) for image classification. In general, the student network had larger values of $N_{\textrm{point}}^{\textrm{fg}}$, $\lambda$, $\rho$, and smaller values of $N_{\textrm{point}}^{\textrm{bg}}$, $D_{\textrm{mean}}$, $D_{\textrm{std}}$ than the baseline network, which verified Hypotheses 1-3.



Comparisons between the student network (S) and the baseline network (B) for the question answering task and the sentiment classification task, respectively. Metrics were evaluated at the last hidden layer of the BERT model, which verified Hypotheses 1-3.



Comparisons between the student network (S) and the baseline network (B) for the classification of 3D point clouds. In general, Hypotheses 1-3 were verified.


Comparisons between the student network (S) and the baseline network (B) for image classification on the MSCOCO dataset. Metrics were evaluated at $\textrm{FC}_{3}$ layer.




\subsection{Verification of Hypothesis 1}
According to Hypothesis 1, a well-trained teacher network was supposed to encode more foreground knowledge points than the student network and the baseline network. 
Consequently, a distilled student network was supposed to model more foreground knowledge points than the baseline network.
It is because the teacher network was usually trained using a large number of training data, and achieved superior performance to the baseline network.
In this way, this well-trained teacher network was supposed to encode more foreground knowledge points than the baseline network. 
Knowledge distillation forced the student network to mimic the teacher network.
Hence, the student network was supposed to model more foreground knowledge points than baseline network.

$\bullet\quad$\textbf{Quantification of knowledge points in the teacher network, the student network and the baseline network.}
Here, we compared knowledge points encoded in the teacher network, the student network, and the baseline network, and verified the above hypothesis.
We learned a VGG-16 model from scratch as the teacher network using the ILSVRC-2013 DET dataset or the CUB200-2011 dataset towards image classification. 
Data augmentation was used to boost the performance of the teacher network.
Table compares the number of foreground knowledge points $N_{\textrm{point}}^{\textrm{fg}}$ learned by the teacher network, the baseline network, and the student network.
For fair comparisons, the student network had the same architecture as the teacher network and the baseline network according to Section.

Table shows that the teacher network usually encoded more foreground knowledge points $N_{\textrm{point}}^{\textrm{fg}}$ and a higher ratio $\lambda$ than the student network.
Meanwhile, the student network often obtained larger values of $N_{\textrm{point}}^{\textrm{fg}}$ and $\lambda$ than the baseline network.
In this way, the above hypothesis was verified.
There was an exception when $N_{\textrm{point}}^{\textrm{fg}}$ was measured at the $\textrm{FC}_{2}$ layer of the VGG-16 model on the ILSVRC-2013 DET dataset.
The teacher network encoded fewer foreground knowledge points than the student network, because this teacher network had a larger average background entropy value $\overline{H}$  than the student network.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


$\bullet\quad$\textbf{Comparing metrics of $N_{\textrm{point}}^{\textrm{fg}}$, $N_{\textrm{point}}^{\textrm{bg}}$ and $\lambda$ to verify Hypothesis 1.}
Unlike the previous subsection learning the teacher network from scratch, in this subsection, we compared $N_{\textrm{point}}^{\textrm{fg}}$, $N_{\textrm{point}}^{\textrm{bg}}$ and $\lambda$ between the student network and the baseline network when using a more sophisticatedly trained teacher network.
In other words, this teacher network was pre-trained on the ImageNet dataset, and then fine-tuned using the ILSVRC-2013 DET dataset, the CUB200-2011 dataset, or the Pascal VOC 2012 dataset. 
This is a more common case in real applications.


Based on the information discarding $\{H_{i}\}$, we visualized image regions in the foreground that corresponded to foreground knowledge points, as well as image regions in the background that corresponded to background knowledge points in Figure~\ref{fig4}, where these knowledge points were measured at the $\textrm{FC}_{1}$ layer of the VGG-11 model.
In this scenario, Hypothesis 1 was also successfully verified.
Moreover, for tasks of image classification, natural language processing, and 3D point cloud classification, 
Table validated Hypothesis 1.
Very few student networks in Table encoded more background knowledge points $N_{\textrm{point}}^{\textrm{bg}}$ than the baseline network. 
It is because teacher networks in this subsection were either pre-trained or trained using more samples, which encoded knowledge points far more than necessary.
In this way, student networks distilled from these well-trained teacher network learned more unnecessary knowledge for inference, thereby leading to a larger $N_{\textrm{point}}^{\textrm{bg}}$ value than the baseline network.



Note that as discussed in Section, knowledge distillation had two different utilities.
The utility of distilling from the low-dimensional network output was mainly to select confident training samples for learning, with very little information on how the teacher network encoded detailed features.
Whereas, the utility of distilling from  high-dimensional intermediate-layer features was mainly to force the student network to mimic knowledge points of the teacher network.
Hence, in this paper, we mainly explained knowledge distillation from high-dimensional intermediate-layer features.


To this end, in Table, we mainly focused on distillation from intermediate-layer features.
Nevertheless, we conducted another experiment to verify that the utility of distilling from relatively low-dimensional network output was to select confident samples and ignore unconfident samples.
Specifically, we distilled the student network from the $10-$dimensional final output of the teacher network for the classification of the top-10 largest categories in the MSCOCO dataset.
Results in Table illustrated the difference between the two utilities of knowledge distillation, to some extent.
For distilling from the 200-dimensional output for the classification on the CUB200-2011 dataset in Table, the Hypothesis 1 was verified, because the network output with $200$ dimensions encoded relatively rich information to force the student network to mimic knowledge points of the teacher network, which reflected the first utility of knowledge distillation.
Whereas, when the network output had very few dimensions, such as 10-category classification on the MSCOCO dataset in Table,  the student network tended to encode both fewer foreground knowledge points and fewer background knowledge points than learning from scratch.
This phenomenon verified the second utility of sample selection.




Additionally, unlike $\textrm{FC}$ layers, convolutional layers were usually not sufficiently fine-tuned due to their depth, when the teacher networks were first pre-trained on the ImageNet dataset for 1000-category classification, and then were fine-tuned using the CUB200-2011 dataset or the Pascal VOC 2012  dataset.
In this scenario, convolutional layers of the teacher network might encode some noisy features, such as features pre-trained for massive unrelated ImageNet categories.
This might violate the first requirement for the knowledge distillation~\textit{i.e.,} the teacher network was supposed to be well optimized for the same task as the student network.
Hence, in order to analyze the convolutional layer in a stricter manner, we conducted another experiment.
Specifically, we fine-tuned the teacher network on the Tiny ImageNet dataset, which was much larger and already had contained sufficient
training images to ensure that features in high convolutional layers were sophisticatedly fine-tuned. 
Table shows that most hypotheses were verified, except that the student network might encode more background knowledge points than the baseline network.
It was because the teacher network encoded significantly more foreground knowledge points in convolutional layers than the baseline network. 
As a cost, the teacher network also encoded a bit more background knowledge points than the baseline network. 
Therefore, the student network encoded much more foreground knowledge points than the baseline network ($3.9$ more foreground knowledge points on average), but just increased background knowledge points by $1.1$.
Nevertheless, the student network still exhibited a larger ratio of foreground knowledge points than the baseline network.
We considered this phenomenon was still reasonable, which had been explained above.



\textbf{Correlation between the quality of knowledge points and classification performance.}
We conducted experiments to check whether the DNN encoding a larger ratio of foreground knowledge points $\lambda$ usually achieved better classification performance, which has been discussed in Section.
To this end, we used the aforementioned student network to describe how the ratio $\lambda$ changes in different epochs of the training process, which was distilled from $\textrm{FC}_1$ layer of the teacher network on the CUB200-2011 dataset for object classification.
Figure shows that DNNs with a larger ratio of task-related knowledge points often exhibited better performance.




Comparison of {\small{$N_{\textrm{point}}^{\textrm{fg}}$}}, {\small{$N_{\textrm{point}}^{\textrm{bg}}$}} and all knowledge points {\small{$N_{\textrm{point}}^{\textrm{all}}= N_{\textrm{point}}^{\textrm{fg}}+ N_{\textrm{point}}^{\textrm{bg}}$}} between fine-tuning a pre-trained VGG-16 network and learning a VGG-16 network from scratch on the Tiny-ImageNet dataset. Metrics were measured at the highest convolutional layer. The fine-tuning process made the DNN encode new foreground knowledge points more quickly and be optimized with fewer detours than learning from scratch.




Comparisons between the student network (S) and the baseline network (B) for image classification on the Tiny-ImageNet dataset. Metrics were evaluated at $\textrm{Conv}$ layer, where Hypotheses 1-3 were verified, to some extent.




\subsection{Verification of Hypothesis 2}
For Hypothesis 2, we assumed that knowledge distillation made the student network learn different knowledge points simultaneously. To this end, we used metrics $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ to verify this hypothesis.

For image classification,
Table \ref{tab:image class} shows that values of $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ were usually smaller than those of the baseline network, which verified Hypothesis 2.
Notice that there exists a very few failure cases. For example, the $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ were measured at the $\textrm{FC}_{1}$ layer of  AlexNet or at the $\textrm{Conv}$ layer of VGG-11. 
It is because both the AlexNet model and the VGG-11 model had relatively shallow network architectures.
When learning from raw data, DNNs with shallow architectures would be easier to learn more knowledge points with less overfitting.


For NLP tasks (question answering and sentiment classification) and the classification of 3D point clouds, 
Table show that the student network had smaller values of $D_{\textrm{mean}}$ and $D_{\textrm{std}}$ than the baseline network, respectively, which successfully verified Hypothesis 2.






\subsection{Verification of Hypothesis 3}
Hypothesis 3 assumed that knowledge distillation made the student network optimized with fewer detours than the baseline network.
The metric $\rho$ measuring the stability of optimization directions was used to verify this hypothesis.


For image classification, natural language processing, and 3D point cloud classification,
Tables show that the student network usually had a larger $\rho$ value than the baseline network, which verified Hypothesis 3.
However, there was few failure cases.
When measuring $\rho$ by AlexNet and VGG-11, shallow architectures of these two networks lead to failure cases (please see discussions in Section~\ref{Verification of Hypothesis 2}).
There was also another failure case when we used the PointNet++ model to measure $\rho$, because this model was discriminative enough.
In this way, this PointNet++ model could make inferences based on a few knowledge points.




\subsection{Analysis of fine-tuning process}
We further checked whether knowledge points could be used to analyze other classic transfer-learning methods.
Here, we focused on fine-tuning a well-trained DNN on a new dataset.
Specifically, we conducted experiments to explore how the fine-tuning process guided the DNN to encode new knowledge points, where we fine-tuned a pre-trained VGG-16 network  on the Tiny ImageNet dataset.
Besides, we also trained another VGG-16 network from scratch on the same dataset  for comparison.
Figure shows that the fine-tuning process made the DNN learn new knowledge points in the foreground more quickly and be optimized with fewer detours than learning from scratch,~\textit{i.e.,} the fine-tuned DNN discarded fewer temporarily learned knowledge points.






\section{Conclusion and discussions}
This paper provides a new perspective to explain knowledge distillation from intermediate-layer features,
\textit{i.e.} quantifying knowledge points encoded in the intermediate layer of a DNN.
We propose three hypotheses on the mechanism of knowledge distillation, and design three types of metrics to verify these hypotheses in the scenario of different classification tasks.
Compared to learning from scratch, knowledge distillation ensures the DNN to encode more knowledge points, learn different knowledge points simultaneously, and optimize with fewer detours.
Note that the learning procedure of DNNs cannot be precisely divided into the learning phase and the discarding phase. In each epoch, the DNN may simultaneously learn new knowledge points and discard old knowledge points irrelevant to the task. Thus, the target epoch $\hat{m}$ in Figure is just a rough estimation of the division of two learning phases.


